Innocent Strategies are Sheaves over Plays---Deterministic, Non-deterministic and Probabilistic Innocence

Although the HO/N games are fully abstract for PCF, the traditional notion of innocence (which underpins these games) is not satisfactory for such language features as non-determinism and probabilistic branching, in that there are stateless terms that are not innocent. Based on a category of P-visible plays with a notion of embedding as morphisms, we propose a natural generalisation by viewing innocent strategies as sheaves over (a site of) plays, echoing a slogan of Hirschowitz and Pous. Our approach gives rise to fully complete game models in each of the three cases of deterministic, nondeterministic and probabilistic branching. To our knowledge, in the second and third cases, ours are the first such factorisation-free constructions.

==> plays-behavs.tex <==
%!TEX root = main.tex
\section{Plays and normal terms}
In game semantics, a term is interpreted as a strategy, i.e.\ a set of \emph{plays} that satisfies some conditions.  By the Taylor expansion followed by  normalisation, a term is transformed into a poly-term, which is characterised by a set (called the \emph{support} of the poly-term) of \emph{normal simple terms}.  In this section, we show that plays and normal simple terms describe different perspectives of the same mathematical objects.  \tk{TODO: check the terminology of Taylor expansion.}

%% In the theory of B\"ohm trees, a term \( M \) can be represented by a set of finite approximants of the B\"ohm tree of \( M \), i.e.\ \( \{ p \mid p \le \mathrm{BT}(M) \} \).  Similarly, a term is interpreted as
%% \begin{itemize}
%% \item a collection of \emph{plays} in game semantics,
%% \item a collection of \emph{normal simple terms} via Taylor expansion, and
%% \item a collection of \emph{types} via an intersection type system.
%% \end{itemize}
%% This section show that these notions describe different perspectives of the same mathematical objects, establishing categorical equivalences between them.

%% This section shows that the game semantics notion of \emph{plays} is equivalent to the notion of \emph{resource terms} \lochanged{in the sense of Ehrhard and Regnier \cite{Ehrhard2008}}. \lo{We should clarify which resource lambda calculus we mean, as there are several in the literature. Is \cite{Ehrhard2008} the best reference?} This equivalence is the basis of the development in subsequent sections.

% \tk{ASIDE: I would like to say that plays and resource terms describe the same thing from a bit different point of view, and I am looking for ``elegant words'' to express this :-)} \lo{What about: Plays and resource terms describe different perspectives of the thing / same mathematical objects.} \tk{Thanks.}

Specifically, we shall define a category of plays and a category of normal simple terms, and establish an equivalence of the categories.

\tk{NOTE: If the interactions in the calculus may cause \emph{infinite chattering}, then the definition of plays (or interaction sequences) below seems incorrect.  Notice that the independent O-moves are (conceptually) asked \emph{concurrently} and thus we should allow interactions having more than one infinite chattering in parallel.  A simple way to overcome the problem is to use tree (or more abstract) representation of plays, instead of the sequential representation in which only the linearly ordered causalities can be expressed.}

\subsection{Plays}
The plays are the most basic object in HO/N game semantics.  Basically they are sequences of moves, representing messages from Opponent and responses by Proponent.  The plays have been considered to form a poset by the prefix ordering, which expresses the progress of the dialogue game between Opponent and Proponent.  That means, when the current play \( s \) is followed by an Opponent message \( m^{\OO}_1 \) and by the Proponent response \( m^{\PP}_2 \), the resulting play is \( s\,m^{\OO}_1\,m^{\PP}_2 \), of which \( s \) is a prefix.  Similarly, if this play is followed by another Opponent message \( m^{\OO}_3 \) and by the Proponent response \( m^{\PP}_4 \), we have \( s\,m^{\OO}_1\,m^{\PP}_2\,m^{\OO}_3\,m^{\PP}_4 \).

\tk{Polish this paragraph.}
However this sequential structure of plays has too much information and some different plays cannot be distinguished by innocent strategies.  For instance, provided that the Opponent message \( m^{\OO}_3 \) is valid at \( s \) already, we have another play \( s\,m^{\OO}_3\,m^{\PP}_4\,m^{\OO}_1\,m^{\PP}_2 \) indistinguishable \tk{Make clear in what sense} from the above play.  But this fact is not reflected to the structure of plays in the standard game semantics.

We consider another kind of extensions:
\begin{enumerate}
\item \( s \)
\item \( s\,m_3^{\OO}\,m_4^{\PP} \)
\item \( s\,m_1^{\OO}\,m_2^{\PP}\,m_3^{\OO}\,m_4^{\PP} \)
\end{enumerate}
Notice that a consecutive moves \( m_1^{\OO}\,m_2^{\PP} \) is inserted in the middle, instead of the tail.  Since innocent strategies cannot distinguish the order of Opponent messages (unless the response to one justifies another), this kind of extension of plays can be justified.

If \( m\,n \) is a valid play, then \( m\,n\,m\,n \) (repeating the same dialogue twice) is also a valid play.  We write this play as \( m_1\,n_1\,m_2\,n_2 \) in order to distinguish the different occurrences of \( m \) and of \( n \).  If we allow to add a PO consecutive moves anywhere, there are two ways to extend \( m\,n \) to \( m_1\,n_1\,m_2\,n_2 \): identifying \( m \) with \( m_1 \) and \( n \) with \( n_1 \) and adding \( m_2\,n_2 \), or identifying \( m \) with \( m_2 \) and \( n \) with \( n_2 \) and adding \( m_1\,n_1 \) at the head.  By properly distinguishing these two extensions, the plays no longer forms a poset but a category, whose objects are plays and a morphism \( f : s \to t \) describes that \( t \) is an extension of \( s \) and how to extend.

Notice the essential use of the innocence in defining morphisms of the category.  If the strategy is not innocent, adding moves at the head is harmful.  So this category should be called the \emph{category of innocent plays}.  This name suggest, for instance, the category of \emph{single-threaded plays} makes sense.

In this subsection, we introduce a novel structure meaning the progress of the game, by which plays are regarded as objects of a category.

We employ a very concrete representation of arenas in which arenas are \emph{ordered} {forests} (i.e.~the childen of each node, as well as the root nodes, are linearly ordered). The order is used to express the order of arguments in the term representation.

\lo{Let $\Nat = \makeset{1, 2, \ldots}$}

\begin{definition}[Arena]
An \emph{(ordered) {forest}} \( M \subseteq \Nat^+ \) is a nonempty subset of nonempty sequences which satisfies
\begin{inparaenum}[(1)]
\item prefix-closure: \( \pi \, k \in M \) implies \( \pi \in M \) for every \( \pi \in \Nat^+ \), and 
\item order-closure: \( \pi \, k \in M \) and \( 1 \leq k' \leq k \) implies \( \pi \, k' \in M \).
\end{inparaenum}  
An \emph{arena} is just a finite (ordered) {forest}.  Given an arena \( M \), the \emph{ownership function} \( \lambda_M : M \to \{ \PP, \OO \} \) is defined by \( \lambda_M(\pi) := \OO \) iff the length of \( \pi \) is odd, and the \emph{enabling relation} \( {\vdash_M} \subseteq (M \uplus \{ \star \}) \times M \) is defined by 
\begin{inparaenum}[(i)]
\item \( \star \vdash_M \pi \) iff the length of \( \pi \) is one, and 
\item \( \pi \vdash_M \pi' \) iff \( \pi' = \pi \, k \) for some \( k \in \Nat \). 
\end{inparaenum} 
An element of \( M \) is called a \emph{move}. A move \( m \in M \) is \emph{initial} if \( \star \vdash m \).  It is a \emph{P-move} if \( \lambda(m) = \PP \); otherwise it is an \emph{O-move}.
\end{definition}
It is obvious that \( (M, \lambda_M, {\vdash_M}) \) is an arena (in which all moves are questions) in the standard sense (as in \cite{HylandO00}).  We use metavariable \( A \) for arenas of this form.

\tkchanged{Unlike the standard formalisation, in which notions such as justified sequences and plays are parametrised by arenas, we parametrise them by a pair of arenas \( (A, B) \), corresponding to the exponential arena \( A \Rightarrow B \) in the standard formalisation.  This change simplifies some definitions.}
\tk{I have removed a condition requiring justified sequences are of even length.}
\begin{definition}[Arena pair]
Let \( A = (\Moves[A], \lambda_A, {\vdash_A}) \) and \( B = (\Moves[B], \lambda_B, {\vdash_B}) \) be arenas.  The \emph{moves of \( (A, B) \)} is the disjoint union of moves, say \( \Moves[A, B] := \Moves[A] + \Moves[B] \).  We define \emph{P-moves} by \( \PMoves[A, B] := \OMoves[A] + \PMoves[B] \) and \emph{O-moves} by \( \OMoves[A, B] := \PMoves[A] + \OMoves[B] \).  For \( m, m' \in \Moves[A, B] \), we write \( m \Vdash_{A, B} m' \) \lo{@Takeshi: By $\Vdash_{A, B}$ do you mean $\vdash_{A, B}$? In Definition~\ref{def:justified_sequence}, for example, you use $\vdash_{A, B}$ rather than $\Vdash_{A, B}$.}just if either
\begin{inparaenum}[(1)]
\item \( m, m' \in \Moves[A] \) and \( m \vdash_{A} m' \), or
\item \( m, m' \in \Moves[B] \) and \( m \vdash_{B} m' \), or
\item \( \star \vdash_{B} m \in \Moves[B] \) and \( \star \vdash_{A} m' \in \Moves[A] \).
\end{inparaenum}
Notice that an initial move of \( A \) may be enabled by more than one or no moves. \lo{I find the preceding sentence somewhat confusing. Did you mean to say: ``Notice that in a justified sequence / play, different occurrences of an initial move of $A$ may be \emph{justified} by different initial moves of $B$.''} We write \( \star \vdash_{A, B} m \) just if \( \star \vdash_{B} m \in \Moves[B] \). 
\end{definition}



%\tk{@Luke: I have largely changed the definition.  20/Jun/2014} \lo{Noted - thanks.}

\lo{? We introduce shorthand: $[n] = \makeset{1, \ldots, n}$ and $[n]_0 = \makeset{0, 1, \ldots, n}$. I prefer $[n]$ to $[1; n]$.}  \tk{You are right.  Sorry for forgetting to define the notation formally.  The reason I changed the notation is that the lower side \( [n, m] \) is \( 1 \) in all but a few exceptional cases.}

\begin{definition}[Justified sequence]\label{def:justified_sequence}
Let \( (A, B) \) be a pair of arenas.  A \emph{justified sequence of \( (A, B) \)} is a finite sequence of moves equipped with justification pointers.  Formally it is a pair of functions \( s : [n] \to \Moves[A, B] \) and \( p : [n] \to [n]_0 \) (for some \( n \)) such that
\begin{itemize}
\item \( p(k) < k \) for every \( k \in [n] \), and
\item \( p \) respects the enabling relation: \( p(k) \ne 0 \) implies \( s(p(k)) \vdash_{A, B} s(k) \), and \( p(k) = 0 \) implies \( \star \vdash_{A, B} s(k) \).
\end{itemize}
As usual, by abuse of notation, we often write \( m_1 \, ßm_2 \dots m_n \) for a justified sequence such that \( s(i) = m_i \) for every \( i \), leaving the justification pointers implicit.  Further we use \( m \) and \( m_i \) as metavariables of \emph{occurrences} of moves in justified sequences.  We write \( m_i \curvearrowleft m_j \) if \( p(j) = i > 0 \) and \( \star \curvearrowleft m_j \) if \( p(j) = 0 \). We call \( m_i \) the \emph{justifier of \( m_j \)} when \( m_i \curvearrowleft m_j \).
\end{definition}

It is convenient to relax the domain \( [n] \) of justified sequences to arbitrary linearly-ordered finite sets such as a subset of \( [1;n] \).  For example, given a justified sequence \( (s: [n] \to \Moves, p : [n] \to [n]_0) \), consider a subset \( I \subseteq [1;n] \) that respects the justification pointers, i.e.~\( k \in I \) implies \( p(k) \in I \cup \{ 0 \} \).  Then the restriction \( (s{|_I} : I \to \Moves, p{|_I} : I \to \{ 0 \} \cup I) \) is a justified sequence in the relaxed sense.  Through the unique monotone bijection \( \alpha : I \to [n'] \), we identify the restriction with the justified sequence in the narrow sense. \lo{}

A justified sequence is \emph{alternating} if \( s(k) \in \OMoves[A,B] \) iff \( k \) is odd (so \( s(k) \in \PMoves[A, B] \) iff \( k \) is even).

\begin{definition}[P-View/P-visibility]
Let \( m_1 \dots m_n \) be an alternating justified sequence.  Its \emph{P-view} \( \View{m_1 \dots m_n} \) (or simply \emph{view}) is a subsequence defined inductively by:
\begin{align*}
  \View{m_1 \dots m_n} &:= \View{m_1 \dots m_{n-1}}\,m_n &\textrm{(if \( m_n \in \PMoves \))} \\
  \View{m_1 \dots m_n} &:= m_n &\textrm{(if \( \star \curvearrowleft m_{n} \in \OMoves \))} \\
  \View{m_1 \dots m_n} &:= \View{m_1 \dots m_k} \, m_n &\textrm{(if \( m_k \curvearrowleft m_n \in \OMoves \)).}
\end{align*}
(Note that \( n \) is even by definition, and thus \( m_{n} \) is a P-move and \( m_{n-1} \) is an O-move.)  \tkchanged{More formally, given an alternating justified sequence \( s \) of length \( n \), its view is a subset \( I \subseteq [n] \).  The above equation gives the restriction of \( s \) to \( I \).  A view is, in general, not a justified sequence since the justifier of a move may be removed.}

Let \( m_k \) be a P-move in the sequence.  Its justifier is said to be \emph{P-visible} (or simply \emph{visible}) if it is in \( \View{m_1 \dots m_k} \).  An alternating justified sequence is \emph{P-visible} (or simply \emph{visible}) \lo{@Takeshi: I ß∫suggest that we always say P-visible (i.e.~we never drop the P) whenever P-visible is intended, to avoid any confusion. It is good to be explicit since the situation here is asymmetric: a play is required to satisfy P- but not O-visibility.} if the justifier of each P-move occurrence in \( s \) is P-visible.
\end{definition}

\begin{definition}[Play]
An alternating justified sequence \lochanged{over a pair $(A, B)$ of arenas} is a %\emph{legal play} (or simply \emph{play}) 
\lochanged{\emph{play} just if} it is visible and its last move is a P-move. \lo{I think it is perfectly fine to define ``play'' and not mention ``legal play'', unless we anticipate working with different and weaker notions of play.}
\end{definition}


\begin{remark}
In contrast to the standard definition of %legal 
play in innocent game semantics, we do not require \emph{O-visibility} because 
\begin{inparaenum}[(1)]
\item O-visibility is not preserved by the morphisms defined below, and 
\item a justified sequence corresponding to a term is not O-visible in general. 
\end{inparaenum} 
Note also that a play may have several initial moves, i.e.~we do not assume \emph{well-openness}.
\end{remark}

\begin{definition}
\tkchanged{Let \( s \) be an alternating justified sequence of \( (A, B) \).  Let \( m_1 \, m_1' \, m_2 \, m_2' \) be consecutive O-P pairs in \( s \), i.e.~\( s = t\,m_1\,m_1'\,m_2\,m_2'\,t' \), where \( m_1 \) and \( m_2 \) are O-moves. We say that the pairs are \emph{exchangeable} if the justifier of \( m_2 \) is \emph{not} \( m_1' \).  The \emph{exchanged sequence} \( s' \) is defined by \( s' := t\,m_2\,m_2'\,m_1\,m_1'\,t' \) (in which the justification pointers are modified accordingly).  More formally, let \( (s : [n] \to \Moves, p : [n] \to [n]_0) \) be an alternating justified sequence.  A consecutive O-P pairs is represented by an odd number \( k \) such that \( k+3 \in [n] \).  It is exchangeable if \( p(k+2) \neq k+1 \).  Let \( f : [n] \to [n] \) be the function defined by:
\[
  f(i) = \left\{\begin{array}{ll}
    k+2 & \textrm{(if \( i = k \))} \\
    k+3 & \textrm{(if \( i = k+1 \))} \\
    k   & \textrm{(if \( i = k+2 \))} \\
    k+1 & \textrm{(if \( i = k+3 \))} \\
    i   & \textrm{(otherwise).}
  \end{array} \right.
\]
Then \( f \circ f \) is the identity function.  The exchanged sequence is \( (s \circ f, \hat{f} \circ p \circ f) \), where \( \hat{f} : [n]_0 \to [n]_0 \) is defined by \( \hat{f}(0) = 0 \) and \( \hat{f}(i) = f(i) \) if \( (i \neq 0) \).
}
\end{definition}
\lo{@Takeshi: What do you think of the following proposal? Instead of saying ``a consecutive pair of O-P pairs is exchangeable'', I suggest that we say ``an adjacent pair of non-interfering O-P pairs''. Instead of ``exchanging'' such a pair, I suggest we say ``commuting''. Reasons: (i) It is generally good to avoid repetition (as in ``exchanging the exchangeable''). (ii) Here ``non-interfering'' is arguably more suggestive than ``exchangeable''.}

Unlike the words, exchangeable pairs in an alternating justified sequence is not always exchangeable: consider the case if \( m_2' \) is justified by \( m_1 \), in which \( m_2' \) in the exchanged sequence is not well-justified.  P-visibility is the condition that ensures exchangeable pairs are in fact exchangeable.  Furthermore the converse also holds.
\begin{lemma}\label{lem:exchange-imply-visibility}
Let \( P \) be a set of even-length alternating justified sequences of \( (A, B) \).  Suppose that \( P \) is closed under exchanges, i.e.~for every sequence \( s \in P \) and every exchangeable pairs in \( s \), the exchanged sequence is also in \( P \).  Then all the moves in \( P \) are P-visible, and hence they are plays.
\end{lemma}
\begin{proof}
Let \( s = m_1 \dots m_n \in P \) and \( m_k \) be a P-move occurrence in \( s \).  By exchanging pairs as much as required, we can reach a sequence, say \( s' = m'_1 \dots m'_n \), such that \( m_l \) is the move corresponding to \( m_k \) in \( s \) and \( m'_{2i} \curvearrowleft m'_{2i+1} \) for every \( 2i < l \).  This means that \( \PView{m_1 \dots m_k} = m_1 \dots m_k \) and hence the justifier of \( m_k \) is in the view.  Since P-visibility is preserved and reflected by the exchange (see Lemma~\ref{lem:exchange-preserve-visibility} below), this means that \( s \) is P-visible.
\end{proof}

\begin{lemma}\label{lem:exchange-preserve-visibility}
Let \( s \) be an alternating sequence and let $t$ be obtained from $s$ by exchanging an exchangeable consecutive O-P pair. Then \( s \) is \lochanged{P-visible} iff \( t \) is \lochanged{P-visible}. \lo{@Takeshi: I suggest that we replace visible by P-visible.}
\end{lemma}
\begin{proof}
Easy.  \tk{TODO: write down}
\end{proof}

A play can be considered as a finite sequence of \emph{pairs} of consecutive O-moves and P-moves.

\begin{definition}[Morphism between plays]\label{def:play-morphism}
Let \( m_1 \dots m_n \) and \( m'_1 \dots m'_{n'} \) be plays of length \( n \) and \( n' \), respectively.  A \emph{morphism between plays} is an injection \( f : [n] \to [n'] \) such that for every \( k \in [n] \)
\begin{enumerate}[(i)]
\item \( m_k = m'_{f(k)} \) (as moves),
\item \( m_i \curvearrowleft m_k \) implies \( m'_{f(i)} \curvearrowleft m'_{f(k)} \) (and similarly for \( \star \curvearrowleft m_k \)), and
\item if an O-move \( m_k \) is followed by a P-move \( m_{k+1} \), then \( m'_{f(k)} \) is followed by \( m'_{f(k+1)} \) \tkchanged{(i.e.\ \( f(2l-1) + 1 = f(2l) \) for all \( l \))}. 
\end{enumerate}
I.e.~a morphism between plays is {an injective} map between the respectives occurrence-sets that preserves moves, justification pointers, and pairs of consecutive O-P moves.
\end{definition}

\begin{example}
%\tkchanged{The exchange \( f \) is a morphism between \( s \) and the exchanged sequence.}
\lochanged{\begin{inparaenum}[(i)]
\item Let $s'$ be obtained from a play $s$ by commuting a non-interfering pair (of consecutive pairs of O-P moves). Then there is an isomorphism $s \to s'$. It follows that there is an isomorphism $s \to s'$ if, and only if, $s'$ is obtainable from $s$ by performing a sequence of commutation of adjacent pairs of non-interfering O-P pairs.
\item For plays \( s \) and \( s' \), we write \( s \le s' \) to mean \( s \) is a prefix of \( s' \). If $s \leq s'$ then there is an obvious morphism $s \to s'$.
\end{inparaenum}}
\end{example}

A bijective map that satisfies the above conditions has a significant property.
\begin{lemma}
\tkchanged{
  Let \( (s : [n] \to \Moves, p : [n] \to [n]_0) \) and \( (s' : [n] \to \Moves, p' : [n] \to [n]_0) \) be justified sequences and \( f : [1;n] \to [1;n] \) be a map that satisfies all the conditions in Definition~\ref{def:play-morphism}.  If \( s \) is a play, then \( s' \) is also a play.
} 
\end{lemma}

\lo{The last sentence can be strengthened to: Then $s$ is a play if, and only if, $s'$ is a play. You have already proved the direction $\Rightarrow$. For the other direction, notice that $f^{-1}$, which is well-defined by assumption, also satisfies Definition~\ref{def:play-morphism}.}

\begin{proof}
Since \( s \) is a play, \( n \) is even.  Since \( f \) maps even numbers to even numbers and odd numbers to odd numbers, alternation of \( s' \) follows from that of \( s \).  So it suffices to check the visibility condition.  Let \( k \in [1;n] \) be an even number and \( j = p(k) \) be its justifier (i.e.~\( s(j) \curvearrowleft s(k) \)).  Since the justifier \( s(j) \) is in the view \( \View{s(1) \dots s(k)} \), there exists a sequence \( l_0, l_1, \dots, l_N \) of odd numbers such that \( j = l_0 \), \( k = l_N + 1 \) and \( s(l_i + 1) \curvearrowleft s(l_{i+1}) \) (for every \( i < N \)).  Let us define that \( l'_i = f(l_i) \) (for every \( i \le N \)).  Then \( f(l_i + 1) = f(l_i) + 1 = l'_i + 1 \) by the condition in Definition~\ref{def:play-morphism}.  Recall that
\[
  s(l_i + 1) \curvearrowleft s(l_{i+1}) \textrm{ implies } s'(f(l_i + 1)) \curvearrowleft s'(f(l_{i+1}))
\]
and hence \( s'(l'_i + 1) \curvearrowleft s'(l'_{i+1}) \).  This means that the justifier \( s'(j') \) of \( s'(k') = s'(l'_N + 1) \) is in the view \( \View{s'(1) \dots s'(l'_N + 1)} \).  This holds for every P-move in \( s' \) since \( f \) is a bijection.
\end{proof}

\begin{remark}
\tk{Meaning of morphisms: if there is \( \varphi : s \to s' \), \( s \) has less information than \( s' \).  If \( \sigma \) is an innocent strategies and \( s' \in \sigma \), then \( s \in \sigma \).}
\end{remark}

\tk{TODO: define \( A \Rightarrow B \).}
\begin{definition}%[Category of plays]
\tkchanged{Let \( A \) and \( B \) be arenas.  The \emph{category \( \CPlay{A, B} \) of plays} has plays of the arena \( A \Rightarrow B \) as objects and as morphisms those defined above.}
\end{definition}

\begin{remark}
\tk{Mellies's observation.  Levy's category.}
\end{remark}


The category \( \mathbb{P}_A \) is an extension of this prefix ordering in the following sense.
\begin{proposition}\label{prop:map-play-char}
If \( s \xrightarrow{f} t \) then there exist a play \( t' \) and an isomorphism \( t' \xrightarrow{g} t \) such that \( s \xrightarrow{f} t = s \xrightarrow{\le} t' \xrightarrow{g} t \). \lochanged{Plainly the converse is also true by composition of morphisms.}
\end{proposition}

Compare with Levy \cite{Levy13} (the slides are available online).

\begin{definition}[Covering family]
A family of morphisms \( \{ f_{\xi} : s_{\xi} \to s \}_{\xi \in \Xi} \) is said to \emph{cover} \( s \) when they are jointly surjective, i.e.\ \( \bigcup_{\xi \in \Xi} \codom(f_{\xi}) = [1;n] \), where \( n \) is the length of \( s \).
\end{definition}

\tk{Some properties of the covering families come here.}



\subsection{Normal terms of the expanded \( \lambda \)-calculus (\( \lambda^{\wedge} \))}
\tk{I notice that the calculus is essentially the same as \( \lambda^{\wedge} \) and its type system (Curry-Howard) System \( \lambda^{\wedge} \)~\cite{Kfoury2000}, including its implicit indexing strategies.}
\tk{Note that the reduction semantics for the calculus depends on the evaluation strategy.  Notice that a reduction may change the left-to-right ordering on occurrences of the same variable (e.g.\ \( (\lambda x. x \langle y_1 \rangle) \langle y_2 \rangle \red y_2 \langle y_1 \rangle \), where \( y_1 \) and \( y_2 \) are different occurrences of the same variable \( y \)).}
\tk{The reduction of this calculus should be the linear-head reduction.}
\tk{I think that \cite{Kfoury2000} may contain a bug: %bag: The calculus does not seem confluent.  This is because left-to-right ordering on variables are not preserved by reduction.  Consider the term: \( M_0 := (\lambda y. (\lambda x. x \langle y \rangle) \langle y \rangle) \langle a, b \rangle \).  By reducing \( \lambda x \) first, we have
\begin{align*}
  M_0
  &\red (\lambda y. y \langle y \rangle) \langle a, b \rangle \\
  &\red a \langle b \rangle,
\end{align*}
while reducing \( \lambda y \) first results in
\begin{align*}
  M_0
  &\red (\lambda x. x \langle a \rangle) \langle b \rangle \\
  &\red b \langle a \rangle.
\end{align*}
Hence we should not use this calculus as a representation of plays: it seems quite hard to prove the associativity of composition.
}

\tk{NOTE: I remove indexes from the terms.  The indexes are implicitly controlled by the syntax.  That means, for \( \lambda \bar{x}. ({\sf p}_i x)\,A_1\,\dots\,A_n \), it must be the case that \( i \) is less than indexes for \( x \) in \( A_1, \dots, A_n \).  Furthermore we require, for every variable \( x \), indexes appearing in \( A_k \) must be less than those in \( A_{k+1} \). In this way, the index for each occurrence is uniquely determined (provided that the set of indexes is a subset of natural numbers of the form \( [1;N] \) for some \( N \)).} \lo{If the requirement is that each occurrence is uniquely determined, then the (implicit) indices should presumably start from 1 i.e.~the leftmost occurrence should have index 1. If so, then the set of indices of a variable in a term is always $[1;m]$ for some $m$. Am I right?}  \tk{Right.}
\tk{By this representation, one can easily establish the connection between plays and terms.  Another option is to change the representation of plays to fit the indexed-term representation by introducing the notion of indexes to plays (so that each occurrence of moves has its index). Then the composition of plays should be defined using these indexes instead of the sequential structure of plays.  I did not choose this since the definition of plays and their composition (perhaps) look very different from the standard definitions.  This representation of plays resembles \cite{DiGianantonioL13} (although they did not characterise the well-formed partitioned positions (NEED TO CHECK), which correspond to the plays).}

This notion corresponds to the notion of plays (but not exactly the same).  Hence it can be represented by terms in normal form (recall the connection between plays and B\"ohm trees, which is a kind of normal form).

The calculus is essentially the same as the \emph{non-uniform \( \lambda \)-calculus} of Melli\'es~\cite{Mellies2006} \tk{But our calculus is finite and linear.} and \emph{multilinear-visible representation of a (poly-)term} by Ehrhard and Regnier~\cite{Ehrhard2008}.  % \lo{@Takeshi: I can't find the phrase ``multilinear-free representation'' in \cite{Ehrhard2008}. Do you mean ``multilinear-visible''?} \tk{@Luke: Right.  What I referred is the HAL version (i.e. a draft version), in which this notion is called ``multilinear-free representation''.  Thanks.}
\tk{We should mention the work \cite{Mazza12}.}
\emph{Terms} and \emph{lists} are defined by

The calculus is essentially the same as the \emph{non-uniform \( \lambda \)-calculus} of Melli\'es~\cite{Mellies2006} \tk{But our calculus is finite and linear.} and \emph{multilinear-free \lo{multilinear-visible(?)} representation of a (poly-)term} by Ehrhard and Regnier~\cite{Ehrhard2008}.  \lo{@Takeshi: I can't find the phrase ``multilinear-free representation'' in \cite{Ehrhard2008}. Do you mean ``multilinear-visible''?} \tk{@Luke: Right.  What I referred is the HAL version (i.e. a draft version), in which this notion is called ``multilinear-free representation''.  Thanks.} \tk{We should mention the work \cite{Mazza12}.}
\emph{Linear terms} are defined by
\[
\begin{array}{lrlcl}
  \textit{Term}&(\Lambda^{\wedge}_{\nf})\quad&
  M, N &{}::={}& \lambda \bar{x}. y\,T_1\,\dots\,T_k
  \\
  \textit{List}&(\bar{\Lambda}^{\wedge}_{\nf})\quad&
  T, U &{}::={}& \langle M_1, \dots, M_n \rangle \textrm{\qquad(\( n \ge 0 \))}.
\end{array}
\]


The \emph{approximation order} of terms are defined by the following rules.  We are interested in how a term can be embedded into another term.  For example, we distinguish two embedding from \( \langle \lambda x. x\,\langle \rangle\;\rangle \) into \( \langle \lambda y. y \langle e_1, e_2 \rangle,\, \lambda z. z \langle h_1, h_2, h_3 \rangle\;\rangle \), identifying \( x \) with \( y \) and \( z \), respectively.  So we define the approximation relation as a triple, \( \varphi \rhd A \sqsubseteq B \), where \( A \) and \( B \) are terms and \( \varphi \) is a witness describing how to embed.
%
\infrule{
  \forall k \in [1;n].\ T_k \sqsubseteq U_k
}{
  (\lambda \bar{x}. y\,T_1\,\dots\,T_n) \sqsubseteq (\lambda \bar{x}. y\,U_1\,\dots\,U_n)
}
\infrule{
  \exists \vartheta : [1;n] \stackrel{\textrm{injection}}{\longrightarrow} [1;m]
  \qquad
  \forall i \in [1;n].\ M_i \sqsubseteq N_{\vartheta(i)}
}{
  \langle M_1, \dots, M_n \rangle \sqsubseteq \langle N_1, \dots, N_m \rangle
}
%

We are interested not only in whether a term can be embedded into another term, but also in how we can embed and how many way.  This is in parallel to the game semantic category of plays, in which we distinguish the way to embed.  \tk{For example, \( \langle \lam x. x \langle \rangle \rangle \) can be embedded into \( \langle \lam x.x \langle \rangle, \lam x. x \langle x \rangle \rangle \) in two ways.}

A way to achieve this is to introduce a term representation of the above rules.  However we adopt a different approach based on an intersection type system.  This type system will be used for another purpose.

\paragraph{Intersection type assignment}
The syntax of types are given by:
\[
\begin{array}{llcl}
  (\textit{Prime type})\quad&
  A, B &{}::={}& \T \mid A^! \multimap B
  \\
  (\textit{Intersection type})\quad&
  A^!, B^! &{}::={}& A_1 \wedge \dots \wedge A_n
\end{array}
\]
where \( n \ge 0 \).  We write \( \tensorunit \) for the empty intersection.  The intersection of intersection types is defined by:
\[
  (A_1 \!\wedge\! \dots \!\wedge\! A_n) \wedge (B_1 \!\wedge\! \dots \!\wedge\! B_m)
  := A_1 \!\wedge\! \dots \!\wedge\! A_n \!\wedge\! B_1 \!\wedge\! \dots \!\wedge\! B_m.
\]
The intersection is assume to be associative, but not commutative (i.e.~\( A \wedge B \neq B \wedge A \)) nor idempotent (i.e.~\( A \wedge A \neq A \)).  However \( A \wedge B \) is isomorphic to \( B \wedge A \) in a certain sense and this isomorphism plays an important role.  \tk{This isomorphism corresponds to reindexing.  It might be better to point out this and the connection to AJM games or Melli{\'e}s's orbital games.}  We use the metavariables like \( A^! \) and \( B^! \) for intersection types, because the intersection types are finite exponential-free approximations of the exponentials.

The intersection is very closed to the tensor of linear logic \tk{Should I cite something?}, but the intersection does not satisfy the law \( A \wedge B \multimap C \eqty A \multimap B \multimap C \).

A \emph{type environment} is a finite partial function from variables to intersection types, represented by a finite sequence.  The typing rules are listed as follows.
%
\infrule{
  \mathstrut
}{
  x : A \vdash x : A
}
\infrule{
  \Gamma_1 \vdash M : A^! \multimap B
  \qquad
  \Gamma_2 \vdash T : A^!
}{
  \Gamma_1 \wedge \Gamma_2 \vdash M\,T : B
}
\infrule{
  \Gamma, x : A^! \vdash M : B
}{
  \Gamma \vdash M : A^! \multimap B
}
\infrule{
  \forall i \in [1;n].\ \Gamma_i \vdash M_i : A_i
}{
  \Gamma_1 \wedge \dots \wedge \Gamma_n \vdash \langle M_1, \dots, M_n \rangle : A_1 \wedge \dots \wedge A_n
}
%
In the last rule, the tensor of type environments is defined by point-wise tensor.  A derivation is \emph{\( \eta \)-long} if every applications are fully-applied.

\begin{lemma}
Every term \( M \) has a unique \( \eta \)-long derivation.  Hence the map \( M \mapsto (\Gamma \vdash A) \), where \( \Gamma \vdash M : A \) has a \( \eta \)-long derivation, is a well-defined function.
\end{lemma}
\begin{proof}
By induction on the structure of \( M \).  The \( \eta \)-long condition is used to determine the type for variables.
\tk{The relaxed version of this lemma holds for general terms.  The relaxed version ensures only uniqueness of \( \eta \)-long derivation, but not the existence.}
\end{proof}

This lemma encourages us to study the normal terms via types.  As we shall see, this is essentially the GoI interpretation. \tk{Need justification?}

\tk{TODO: some words}
%
\infrule{
  \mathstrut
}{
  \BM \rhd \T \subty \T
}
\infrule{
  \varphi \rhd A^!_1 \subty B^!_1
  \qquad
  \vartheta \rhd A_2 \subty B_2
}{
  (\varphi \multimap \vartheta) \rhd (A^!_1 \multimap A_2) \subty (B^!_1 \multimap B_2)
}
\infrule{
  \varphi : [1;n] \stackrel{\mathrm{injection}}{\longrightarrow} [1;m]
  \qquad
  \forall i \in [1;n].\ \vartheta_i \rhd A_i \subty B_{\varphi(i)}
}{
  (\bigwedge_{i \in [1;n]}^{\varphi} \vartheta_i) \rhd (A_1 \wedge \dots \wedge A_n) \subty (B_1 \wedge \dots \wedge B_m)
}
%
Let \( \Phi \) be a partial map from variables to witnesses.  We write \( \Phi \rhd \Gamma \subty \Gamma' \) if \( \dom(\Phi) = \dom(\Gamma) \) and \( \Phi(x) \rhd \Gamma(x) \subty \Gamma'(x) \) for every \( x \in \dom(\Gamma) \).  We write \( (\Phi \vdash \varphi) \rhd (\Gamma \vdash A) \subty (\Gamma' \vdash A') \) if \( \Phi \rhd \Gamma \vdash \Gamma' \) and \( \varphi \rhd A \subty A' \).

Let \( \Gamma \vdash M : A \) and \( \Gamma' \vdash M' : A' \) and \( (\Phi \vdash \varphi) \rhd (\Gamma \vdash A) \subty (\Gamma' \vdash A') \).  The relation \( (\Phi \vdash \varphi) \rhd (\Gamma \vdash M : A) \sqsubseteq (\Gamma' \vdash M' : A') \) is defined by induction on derivations:
%
\infrule{
  (\Phi[x \mapsto \psi], \varphi) \rhd (\Gamma, x : \vec{A} \vdash M : B) \sqsubseteq (\Gamma', x : \vec{A}' \vdash M' : B')
}{
  (\Phi, (\psi, \varphi)) \rhd (\Gamma \vdash \lam x. M : \vec{A} \multimap B) \sqsubseteq (\Gamma' \vdash \lam x. M' : \vec{A}' \multimap B')
}
\infrule{
  \exists \vartheta \rhd \vec{B} \subty \vec{B}' \\
  (\Phi_1, (\vartheta, \varphi)) \rhd (\Gamma_1 \vdash M : \vec{B} \multimap A) \sqsubseteq (\Gamma'_1 \vdash M' : \vec{B}' \multimap A')
  \\
  (\Phi_2, \vartheta) \rhd (\Gamma_2 \vdash T : \vec{B}) \sqsubseteq (\Gamma'_2 \vdash T' : \vec{B}')
}{
  (\Phi_1 \wedge \Phi_2, \varphi) \rhd (\Gamma_1 \wedge \Gamma_2 \vdash M\,T : A) \sqsubseteq (\Gamma'_1 \wedge \Gamma'_2 \vdash M'\,T' : A')
}
\infrule{
  \forall i \in [n].\ (\Phi_i, \varphi_i) \rhd (\Gamma_i \vdash M_i : A_i) \sqsubseteq (\Gamma'_{\vartheta(i)} \vdash M'_{\vartheta(i)} : A'_{\vartheta(i)})
}{
  (\bigwedge_{i \in [n]} \Phi_i, (\vartheta, (\varphi_i)_{i \in [n]})) \\
  \rhd (\bigwedge_{i \in [n]} \Gamma_i \vdash \langle M_i \rangle_{i \in [n]} : \bigwedge_{i \in [n]} A_i) \sqsubseteq (\bigwedge_{j \in [m]} \Gamma'_j \vdash \langle M'_j \rangle_{j = [m]} : \bigwedge_{j = [m]} A'_j)
}
%
\tk{What is the point?}  \tk{Games are based on the sequential structure with justification.  Types are based on the justification structure and sequential structure is captured by the above rules.}

The composition is defined by: \( \BM \circ \BM := \BM \), \( (\varphi' \multimap \vartheta') \circ (\varphi \multimap \vartheta) := (\varphi' \circ \varphi) \multimap (\vartheta' \circ \vartheta) \) and
\[
  (\bigwedge_{j \in [m]}^{\varphi'} \vartheta'_j) \circ (\bigwedge_{i \in [n]}^{\varphi} \vartheta_i) := \bigwedge_{i \in [n]}^{\varphi' \circ \varphi} \vartheta'_{\varphi(i)} \circ \vartheta_i.
\]
The composition can be straightforwardly extended to \( \Phi \rhd \Gamma \subty \Gamma' \) and \( (\Phi \vdash \varphi) \).
\begin{lemma}
Suppose that 
\[
  (\Gamma_1 \vdash M_1 : A_1) \stackrel{\Phi \vdash \varphi}{\longrightarrow}
  (\Gamma_2 \vdash M_2 : A_2) \stackrel{\Phi' \vdash \varphi'}{\longrightarrow}
  (\Gamma_3 \vdash M_3 : A_3).
\]
Then \( (\Phi' \vdash \varphi') \circ (\Phi \vdash \varphi) : (\Gamma_1 \vdash M_1 : A_1) \to (\Gamma_3 \vdash M_3 : A_3) \).
\end{lemma}

Hence they form a category.  \tk{state associativity of the composition.  Existence of the identity is rather trivial.}

For a function \( f : A \to B \), its image is defined by \( \codom(f) := \{ f(a) \mid a \in A \} \).  Let us fix a kind \( \kappa \) and consider the category \( \mathbbm{B}_{\kappa} \).  Assume an object \( e \in \mathbbm{B}_{\kappa} \) and a family of maps \( \{ \varphi^\xi : e^{\xi} \to e \}_{\xi \in \Xi} \).  This family \emph{covers} \( e \) just if the union of the image of \( \varphi_\xi \), as $\xi$ ranges over $\Xi$, is \( e \).  This notion can be formally defined by induction on \( e \):
\begin{itemize}
\item If \( e = \lambda \bar{x}. y\,A_1\,\dots\,A_n \), then for each \( \xi \in \Xi \), we have \( e^{\xi} = \lambda \bar{x}. y\,A^{\xi}_1\,\dots\,A^{\xi}_n \) and \( \varphi^\xi = (\varphi^\xi_1, \dots, \varphi^\xi_n) \).  The family covers \( e \) just if
  \begin{enumerate}
  \item The family is nonempty, and
  \item \( \{ \varphi^{\xi}_k : A^{\xi}_k \to A_k \}_{\xi \in \Xi} \) covers \( A_k \) for every \( k \).
  \end{enumerate}
\end{itemize}
For lists, we define
\begin{itemize}
\item For a list \( A = \langle e_1, \dots, e_n \rangle \), consider the family \( \{ \varphi^{\xi} : A^{\xi} \to A \}_{\xi \in \Xi} \).  We have \( A^{\xi} = \langle e^{\xi}_1, \dots, e^{\xi}_{n^{\xi}} \rangle \) and \( \varphi^{\xi} = (\vartheta^{\xi}, (\varphi^{\xi}_j)_{j \in [1; n^{\xi}]}) \).  This family covers \( A \) just if, for every \( i \in [1;n] \), the family \( \{ \varphi^{\xi}_j : e^{\xi}_j \to e_i \mid \vartheta^{\xi}(j) = i \} \) covers \( e_i \).
\end{itemize}
Notice that this condition implies that \( [1;n] = \bigcup_{\xi \in \Xi} \codom(\vartheta^{\xi}) \).  Otherwise, for \( i \in I - (\bigcup_{\xi \in \Xi} \codom(\vartheta^{\xi}) \), the family \( \{ \varphi^{\xi}_j : e^{\xi}_j \to e_i \mid \vartheta^{\xi}(j) = i \} \) is empty and thus cannot cover \( e_i \).

\tk{TODO: terminology}


\tk{We introduce a simple-type assignment system for normal terms.  The typing rules are listed as follows.}
%
\infrule{
  y :: \delta_1 \to \dots \to \delta_m \to \T \in \Gamma \hfill
  \\
  \forall k \in [1;m].\quad \Gamma, x_1 :: \kappa_1, \dots, x_n :: \kappa_n \vdash A_k :: \delta_k
}{
  \Gamma \vdash \lambda x_1 \dots x_n. y\,A_1\,\dots\,A_m :: \kappa_1 \to \dots \to \kappa_n \to \T
}
\infrule{
  \forall k \in [1;n].\ \Gamma \vdash e_i :: \kappa
}{
  \Gamma \vdash \langle e_1, \dots, e_n \rangle :: \kappa
}
%

\begin{definition}
\tk{Define a category \( \mathbb{B}_{\Gamma, \Delta} \).}  \tk{\( \mathbb{B}_{\kappa} \) is a full subcategory.}
\end{definition}




\subsection{Adjoint equivalence}
We have defined the category of plays \( \mathbb{P}_A \) for an arena \( A \) and the category of terms \( \mathbb{B}_\kappa \) for a kind \( \kappa \).  This subsection establishes an equivalence between \( \mathbb{P}_{\kappa} \) and \( \mathbb{B}_{\kappa} \), where \( \mathbb{P}_{\kappa} \) is the category of plays of the arena corresponding to \( \kappa \).

\subsubsection{From kinds to arenas}
Given a kind \( \kappa \), the set of \emph{paths} \( \mathit{Path}(\kappa) \subseteq \Nat^* \) is a (finite) set defined by:
\(
  \mathit{Path}(\kappa_1 \to \dots \to \kappa_n \to \T) := \{ \varepsilon \} \cup \{ k \, \pi \mid k \in [1;n], \pi \in \mathit{Path}(\kappa_k) \}
\).
The arena \( A(\kappa) \) is defined as \( (\mathit{Path}(\kappa), \lambda, \vdash) \) where
\begin{itemize}
\item \( \lambda(\pi) := \OO \) if the length of \( \pi \) is odd, and
\item \( \pi \vdash \pi' \) when \( \pi' = k \, \pi \) for some \( k \in \Nat \), \( \star \vdash \pi \) when \( \pi = \varepsilon \).
\end{itemize}

\subsubsection{From terms to plays}
We use an alternative representation of plays in which O-moves has pointers and P-moves does not have pointers but have variable name.  So in a sequence the pointer from a P-move labelled \( x \) is the abstraction that introduces the name \( x \), i.e.~a move of the form \( \lambda \bar{y} \) where \( x \in \bar{y} \).
\begin{align*}
  F(\lambda \bar{x}. y\,T_1\,\dots\,T_n) &:= [\lambda \to \T] \bar{x}]\;[y]\; F(T_1)\;\dots\;F(T_n) \\
  F(\langle M_1, \dots, M_n \rangle) &:= F(M_1) \dots F(M_n)
\end{align*}
where in the first expression the initial moves of \( F(T_i) \) points to \( [y] \).  The justification pointer is defined as described above.  The map to a move label is the type for each node, i.e.~\( [\lambda \bar{x}] \mapsto \bar{\kappa} \to \T \) (where \( \bar{\kappa} = \kappa_1 \to \dots \to \kappa_n \) is the sequence of simple types of the variables \( \bar{x} = x_1 x_2 \dots x_n \)) and \( [y] \mapsto \kappa \) (where \( \kappa \) is the simple type for \( y \)).

\tk{Define the morphism part.}

\begin{lemma}
\( F \) is a functor.
\end{lemma}

\subsubsection{From plays to terms}
\tk{TODO: define \( G \).}

\lochanged{We define a functor $G : \cat{P}_\kappa \to \cat{B}_\kappa$ as follows. First the map on objects. In the base case, $G$ maps the empty play to $\anglebra{}$. For the inductive case, take a play $s \, m_1^O \, m_2^P$. Suppose $m^O_1$ is initial, then it follows from P-visibility that $m_2^P$ is justified by $m_1^O$, and so, $G(s \, m_1^O \, m_2^P) := \anglebra{e_1, \ldots, e_n, \lambda \bar{x}.x_i}$ where $G(s) = \anglebra{e_1, \ldots, e_n}$ and $m_2^P$ is the $i$-child of $m_1^O$. Now suppose $m_1^O$ is justified by the move $m_0^P$, which occurs in $s$. By O-justification, we may assume that $G(s) = C[x \, A_1 \ldots A_i \ldots A_m]$ where $C[\,]$ is a term context, $[x] = m_0^P$ (i.e.~$x$ corresponds to $m_0^P$), $m_1^O$ is the $i$-child of $m_0^P$, and $A_i = \anglebra{e_1, \ldots, e_n}$. Then $G(s \, m_1^O \, m_2^P) := C[x \, A_1 \ldots \anglebra{e_1, \ldots, e_n, \lambda \bar{x}.y} \ldots A_m]$ where $[\lambda \bar{x}] = m_1^O$ and $[y] = m_2^P$.}

\lo{Ongoing}

\begin{lemma}
The pair of functors \( F \) and \( G \) forms an adjoint equivalence.  They preserve and reflect the covering families.  \tk{TODO: check the correctness of the terminology.}
\end{lemma}




\subsection{Strategies}
Let \( \CVal \) be a finitely complete category with countable coproducts.  Then a strategy is just a \( \CVal \)-valued sheaf \( \Sheaf(\CPlay{A, B}, \CVal) \), which is a functor \( F : \CPlay{A, B}^{\op} \longrightarrow \CVal \) such that, for every \( s \in \CPlay{A, B} \) and \( S \in J(s) \), the diagram
%% \[\xymatrix@R-0.1cm@C.8cm{
%%   F(s) \ar[r] & {\displaystyle \prod_{f \in S} F(\dom(f))} \ar@<2pt>[r] \ar@<-2pt>[r] & \prod_{f, g \in S} F(\dom(f) \times_{s} \dom(g))
%% }
%% \]
\[
  F(s) \rightarrow \prod_{f \in S} F(\dom(f)) \rightrightarrows \prod_{f, g \in S} F(\dom(f) \times_{s} \dom(g))
\]
is an equaliser.  Here \( F(s) \rightarrow \prod_{f \in S} F(\dom(f)) \) is determined by \( F(f) : F(s) \to F(\dom(f)) \) and the parallel arrows are determined by the projections to the first and the second component of the pullback diagram.  Note that a sieve \( S \) in \( \CPlay{A, B} \) is a finite set and thus the products in the above diagram are finite products.

\tk{Note about comparison lemma?---\( \Sheaf(\CPlay{A, B}, \CVal) \cong \Sheaf(\CView{A, B}, \CVal) \)?  Is it applicable to general sheaves \( \Sheaf(\CPlay{A, B}, \CVal) \) or set-valued sheaves \( \Sheaf(\CPlay{A, B}, \mathbf{Set}) \)?}

\begin{proposition}[View functionality 1]
Let \( F_1, F_2 \in \Sheaf(\CPlay{A, B}, \CVal{V}) \) be sheaves.  If they coincides on views (i.e.~\( F_1 \circ \iota = F_2 \circ \iota \) where \( \iota : \CView{A, B} \hookrightarrow \CPlay{A, B} \) is the inclusion), then they are naturally isomorphic.
\end{proposition}

\begin{proposition}[View functionality 2]
Every functor \( F_0 : \CView{A, B}^{\op} \to \CVal \) from views to \( \CVal \) can be extended to a sheaf \( F \in \Sheaf(\CPlay{A, B}, \CVal) \) (i.e.~\( F \circ \iota = F_0 \)).
\end{proposition}



==> resource-calculus.tex <==
%!TEX root = main.tex
\section{Resource calculus} 
\label{sec:resource-calculus}
This section gives a definition of the resource \( \lambda \)-calculus, which we call \( \lambda^{r} \) in the paper.  The calculus is simply typed.

\subsection{Terms}
\emph{Terms} and \emph{bags} are defined by
\[
\begin{array}{llcl}
  (\textit{Term};\;\Lambda^{r})\quad&
  M, N &{}::={}& x \mid \lambda \bar{x}. M \mid M\,T
  \\
  (\textit{Bags};\;\bar{\Lambda}^{r})\quad&
  T, U &{}::={}& \bag{M_1, \dots, M_n}
\end{array}
\]
where \( n \ge 0 \).  A bag \( \bag{M_1, \dots, M_n} \) means the multiset consisting of \( M_i \)'s and thus \( \bag{M_1, \dots, M_n} = \bag{M_{\sigma(1)}, \dots, M_{\sigma(n)}} \) if \( \sigma \) is a permutation of \( [1;n] \).

We consider only well-typed terms.  The typing rules are listed as follow.
%
\infrule{
  x :: \delta \in \Gamma
}{
  \Gamma \vdash x :: \delta
}
\infrule{
  \Gamma, x :: \delta \vdash M :: \delta'
}{
  \Gamma \vdash \lambda x. M :: \delta \to \delta'
}
\infrule{
  \Gamma \vdash M :: \delta \to \delta'
  \qquad
  \Gamma \vdash T :: \delta
}{
  \Gamma \vdash M\,T :: \delta'
}
%% \infrule{
%%   y :: \delta_1 \to \dots \to \delta_m \to \T \in \Gamma \hfill
%%   \\
%%   \forall k \in [1;m].\quad \Gamma, x_1 :: \kappa_1, \dots, x_n :: \kappa_n \vdash T_k :: \delta_k
%% }{
%%   \Gamma \vdash \lambda x_1 \dots x_n. y\,T_1\,\dots\,T_m :: \kappa_1 \to \dots \to \kappa_n \to \T
%% }
\infrule{
  \forall k \in [1;n].\ \Gamma \vdash M_i :: \kappa
}{
  \Gamma \vdash \bag{M_1, \dots, M_n} :: \kappa
}
%
This type system captures the image of Taylor expansion of type terms in the sense that a term of type \( \delta \) is mapped to a set of \( \lambda^r \)-terms of type \( \delta \) by the Taylor expansion.  This type system does not enjoy ``type safety'', i.e.\ a typed term may get stuck, as we shall see below.  Type safety shall be ensured by a more sophisticated intersection type system.



\subsection{Intersection type system}
We develop an intersection type system in which a derivation represents a successful reduction sequence.  

Intersection types are defined by:
\[
\begin{array}{llcl}
  (\textit{Prime type})\quad&
  A, B &{}::={}& \T \mid A^! \multimap B
  \\
  (\textit{Intersection type})\quad&
  A^!, B^! &{}::={}& A_1 \otimes \dots \otimes A_n
\end{array}
\]
where \( n \ge 0 \).  We write \( \mathbf{1} \) for the empty intersection.  The intersection on intersection types are defined by:
\[
  (A_1 \otimes \dots \otimes A_n) \otimes (B_1 \otimes \dots \otimes B_m) := A_1 \otimes \dots \otimes A_n \otimes B_1 \otimes \dots \otimes B_m.
\]
Hence \( \otimes \) can be considered as an associative operator, but it is not idempotent (i.e.\ \( A \otimes A \neq A \)) nor commutative (i.e.\ \( A \otimes B \neq B \otimes A \)).  However the commutativity law holds up to isomorphism, i.e.\ \( A \otimes B \) is isomorphic to \( B \otimes A \), by the rule introduced below.

%
\infrule{
  \mathstrut
}{
  \T :: \T
}
\infrule{
  A^! :: \delta
  \qquad
  B :: \delta'
}{
  A^! \multimap B \;{}::{}\; \delta \to \delta'
}
\infrule{
  \forall i \in [1;n].\ A_i :: \delta
}{
  A_1 \otimes \dots \otimes A_n :: \delta
}
%




%
\infrule{
  \mathstrut
}{
  () \rhd \T \subty \T
}
\infrule{
  \varphi \rhd A^! \subty B^!
  \qquad
  \vartheta \rhd A' \subty B'
}{
  (\varphi, \vartheta) \rhd (A^! \multimap A') \subty (B^! \multimap B')
}
\infrule{
  \varphi : [1;n] \stackrel{\mathrm{injection}}{\longrightarrow} [1;m]
  \qquad
  \forall i \in [1;n].\ \vartheta_i \rhd A_i \subty B_{\varphi(i)}
}{
  (\varphi, (\vartheta_i)_{i \in [1;n]}) \rhd (A_1 \otimes \dots \otimes A_n) \subty (B_1 \otimes \dots \otimes B_m)
}
%

%
\infrule{
  \mathstrut
}{
  () \rhd \T \osubty \T
}
\infrule{
  \varphi \rhd A^! \psubty B^!
  \qquad
  \vartheta \rhd A' \osubty B'
}{
  (\varphi, \vartheta) \rhd (A^! \multimap A') \osubty (B^! \multimap B')
}
\infrule{
  \varphi : [1;n] \stackrel{\mathrm{injection}}{\longrightarrow} [1;m]
  \qquad
  \forall i \in [1;n].\ \vartheta_i \rhd A_i \osubty B_{\varphi(i)}
}{
  (\varphi, (\vartheta_i)_{i \in [1;n]}) \rhd (A_1 \otimes \dots \otimes A_n) \osubty (B_1 \otimes \dots \otimes B_m)
}
%
%
\infrule{
  \mathstrut
}{
  () \rhd \T \psubty \T
}
\infrule{
  \varphi \rhd \vec{A} \osubty B^!
  \qquad
  \vartheta \rhd A' \psubty B'
}{
  (\varphi, \vartheta) \rhd (A^! \multimap A') \psubty (B^! \multimap B')
}
\infrule{
  \forall i \in [1;n].\ \vartheta_i \rhd A_i \psubty B_{i}
}{
  (\mathrm{id}, (\vartheta_i)_{i \in [1;n]}) \rhd (A_1 \otimes \dots \otimes A_n) \psubty (B_1 \otimes \dots \otimes B_n)
}
%

\begin{lemma}
Every morphism \( \varphi \rhd A \subty B \) is uniquely factorised as \( \varphi = \varphi_\OO \circ \varphi_\PP \) such that \( \varphi_{\OO} \in \OO \) and \( \varphi_{\PP} \in \PP \).
\end{lemma}

\begin{lemma}
A morphism \( \varphi \rhd A \subty B \) can be considered as an IMLL proof of \( A \multimap B \).  Furthermore \( \varphi \neq \varphi' \) as witnesses of refinement, they correspond to different proofs.
\end{lemma}

Prime types and refinement relations (with witnesses) form a category.  The composition of \( \varphi \rhd A \subty A' \) and \( \varphi' \rhd A' \subty A'' \) is \( \varphi' \circ \varphi \rhd A \subty A'' \) defined by: \( () \circ () := () \), \( (\varphi', \vartheta') \circ (\varphi, \vartheta) := (\varphi' \circ \varphi,\ \vartheta' \circ \vartheta) \) and
\[
  (\varphi', (\vartheta_i)_{i \in [1;m]}) \circ (\varphi, (\vartheta_i)_{i \in [1;n]}) = (\varphi' \circ \varphi, (\vartheta'_{\varphi(i)} \circ \vartheta_i)_{i \in [1;n]}).
\]
Here \( \varphi' \circ \varphi \) is the standard composition of functions.

\tk{Since \( (\varphi, (\vartheta_i)_{i \in [1;n]}) \rhd \vec{A} \subty \vec{A}' \), we have \( \vartheta_i \rhd A_i \subty A'_{\varphi(i)} \).  Since \( (\varphi', (\vartheta'_j)_{j \in [1;m]}) \rhd \vec{A}' \subty \vec{A}'' \), we have \( \vartheta'_j \rhd A'_j \subty A''_{\varphi'(j)} \) and thus \( \vartheta'_{\varphi(i)} \rhd A'_{\varphi(i)} \subty A''_{\varphi'(\varphi(i))} \).}

\begin{example}
We have \( \T \subty \T \otimes \T \).  We have two morphisms, say \( \varphi_1 = (\{ 1 \mapsto 1 \}, ()) \) embedding into the left component of the intersection type and \( \varphi_2 = (\{ 1 \mapsto 2 \}, ()) \) embedding into the right component.
\end{example}

We write \( \varphi \rhd A \eqty B \) when \( \varphi \) is invertible, and \( A \eqty B \) when \( \varphi \rhd A \eqty B \) for some \( \varphi \) (i.e.\ \( A \) and \( B \) are isomorphic).  We write \( \varphi \rhd A \oeqty B \) when \( \varphi \rhd A \eqty B \) and \( \varphi \) is in \( \OO \) (then \( \varphi^{-1} \) is also in \( \OO \)).  Similarly for \( \varphi \rhd A \peqty B \).
\begin{lemma}
If \( \varphi \rhd A \subty B \) and \( \varphi' \rhd B \subty A \), then \( A \) and \( B \) are isomorphic (but \( \varphi' \) is not necessarily the inverse of \( \varphi \)).
\end{lemma}

The refinement relation can be extended to type environments: \( \Phi \rhd \Gamma \subty \Gamma' \) when \( \Phi(x) \rhd \Gamma(x) \subty \Gamma'(x) \) for all \( x \in \dom(\Gamma) \).  We define \( \Gamma \otimes \Gamma' \) by \( (\Gamma \otimes \Gamma')(x) := \Gamma(x) \otimes \Gamma'(x) \).
%
\infrule{
  \mathstrut
}{
  x \rhd x : A \vdash x : A
}
\infrule{
  \mathscr{D} \rhd \Gamma, x : \vec{A} \vdash M : B
}{
  (\lambda x. \mathscr{D}) \rhd \Gamma \vdash \lambda x. M : \vec{A} \multimap B
}
\infrule{
  \mathscr{D}_1 \rhd \Gamma_1 \vdash M : \vec{A} \multimap B
  \qquad
  \mathscr{D}_2 \rhd \Gamma_2 \vdash T : \vec{A}
}{
  (\mathscr{D}_1, \mathscr{D}_2) \rhd \Gamma_1 \otimes \Gamma_2 \vdash M\,T : B
}
\infrule{
  \forall i \in [1;n].\ \mathscr{D}_i \rhd \Gamma_i \vdash M_i : A_i
}{
  (\mathscr{D}_i)_{i \in [1;n]} \rhd \bigotimes_{i \in [1;n]} \Gamma_i \vdash \bag{M_i}_{i \in [1;n]} : \bigotimes_{i \in [1;n]} A_i
  \\
  (\mathscr{D}_i)_{i \in [1;n]} \rhd \Gamma_1 \otimes \dots \otimes \Gamma_n \vdash \bag{M_1, \dots, M_n} : A_1 \otimes \dots \otimes A_n
}
\infrule{
  \Phi \rhd \Gamma' \oeqty \Gamma
  \qquad
  \mathscr{D} \rhd \Gamma \vdash M : A
  \qquad
  \vartheta \rhd A \peqty A'
}{
  (\Phi, \mathscr{D}, \vartheta) \rhd \Gamma \vdash M : A'
}
%
\tk{I wrote two representation of the conclusion in the rule for bags.  We should compare them and choose understandable one.}
A witness \( \mathscr{D} \) in the above rules is called a \emph{derivation}.  We write \( \Gamma \vdash M : A \) when \( \mathscr{D} \rhd \Gamma \vdash M : A \) for some derivation \( \mathscr{D} \).
Since \( \bag{M_1, \dots, M_n} = \bag{M_{\sigma(1)}, \dots, M_{\sigma(n)}} \) for every permutation \( \sigma \), we have \( \Gamma \vdash \bag{M_1, \dots, M_n} : \vec{A} \) if and only if \( \Gamma \vdash \bag{M_{\sigma(1)}, \dots, M_{\sigma(n)}} : \vec{A} \).  In general, \( \Gamma \vdash M : A \) if and only if \( \Gamma' \vdash M : A' \) whenever \( \Gamma \eqty \Gamma' \) and \( A \eqty A' \).  \tk{Is this true?  This is highly nontrivial since the current type system only arrows P-rearrangement.}  \tk{This seems true.  This observation is a reminiscent of the work by Melli\'es of ``uniformity by group invariance''~\cite{Mellies2003} (though his paper contains bugs).}

\begin{example}
Let \( \Gamma = a : \T, b : \T \).  We have \( \Gamma \vdash \bag{a, b} : \T \otimes \T \).  We have two derivations: \( (a, b) \rhd \Gamma \vdash \bag{a, b} : \T \otimes \T \) and \( (b, a) \rhd \Gamma \vdash \bag{a, b} : \T \otimes \T \).  Notice that elements in the bag is ordered though the derivation, whereas it is unordered in the term (recall that \( \bag{a, b} = \bag{b, a} \)).  In other words, giving a derivation is equivalent to ordering elements in bags.
\end{example}

\subsubsection{Equivalence of derivations}
\[
  (\mathrm{id}, \mathscr{D}, \mathrm{id}) = \mathscr{D}
\]
\[
  (\Phi, (\Phi', \mathscr{D}, \vartheta'), \vartheta) = ((\Phi; \Phi'), \mathscr{D}, (\vartheta';\vartheta))
\]
\[
  (\{ x \mapsto \varphi^{-1} \}, x, \varphi) = x
\]
where \( f;g := g \circ f \).
\[
  (\mathscr{D}_1, \mathscr{D}_2) = ((\mathrm{id}, \mathscr{D}_1, (\varphi^{-1}, \mathrm{id})), (\mathrm{id}, \mathscr{D}_2, \varphi))
\]
\[
  (\Phi, (\mathscr{D}_i)_{i \in [1;n]}, (\varphi, (\vartheta_i)_{i \in [1;n]})) = ...
\]
We write \( [\mathscr{D}] \) for the equivalence class of derivations.  A derivation is \emph{commutation free} if it does not use the isomorphism rule (i.e.\ if it does not have a subderivation of the form \( (\Phi, \mathscr{D}', \vartheta) \)).

\tk{This equivalence seems more naturally understood by the notion of proof-nets.}
\tk{It might be better to define the equivalence via GoI interpretation.}

\begin{lemma}
Any equivalence class of derivations \( [\mathscr{D}] \) can be uniquely represented by \( (\Phi, \mathscr{E}, \vartheta) \) such that \( \mathscr{E} \) is commutation free, \( \Phi \in \OO \) and \( \vartheta \in \PP \).
\end{lemma}
\begin{proof}
\tk{TODO: check.}
\end{proof}

Assume the notion of an \emph{occurrence} of a prime type \( B \) in type \( A \) or \( \vec{A} \).  A derivation \( \mathscr{D} \rhd \Gamma \vdash M : A \) determines bijections between \( (i) \) covariant occurrences and abstracitons in the term and \( (ii) \) contravariant occurrences and variables in the term.  \tk{TODO: check.  Perhaps we need some assumption like \( \eta \)-long.}


\begin{remark}
The category of normal derivations are equivalent to the category of plays.  The unity of duality of this adjunction is commutation free derivations followed by the contravariant commutation.
\end{remark}





==> terms.tex <==
%!TEX root = main.tex
\section{Term-based Representation}

\subsection{Normal terms of the expanded \( \lambda \)-calculus (\( \lambda^{\wedge} \))}
\tk{I notice that the calculus is essentially the same as \( \lambda^{\wedge} \) and its type system (Curry-Howard) System \( \lambda^{\wedge} \)~\cite{Kfoury2000}, including its implicit indexing strategies.}
\tk{Note that the reduction semantics for the calculus depends on the evaluation strategy.  Notice that a reduction may change the left-to-right ordering on occurrences of the same variable (e.g.\ \( (\lambda x. x \langle y_1 \rangle) \langle y_2 \rangle \red y_2 \langle y_1 \rangle \), where \( y_1 \) and \( y_2 \) are different occurrences of the same variable \( y \)).}
\tk{The reduction of this calculus should be the linear-head reduction.}
\tk{I think that \cite{Kfoury2000} may contain a bug: %bag: The calculus does not seem confluent.  This is because left-to-right ordering on variables are not preserved by reduction.  Consider the term: \( M_0 := (\lambda y. (\lambda x. x \langle y \rangle) \langle y \rangle) \langle a, b \rangle \).  By reducing \( \lambda x \) first, we have
\begin{align*}
  M_0
  &\red (\lambda y. y \langle y \rangle) \langle a, b \rangle \\
  &\red a \langle b \rangle,
\end{align*}
while reducing \( \lambda y \) first results in
\begin{align*}
  M_0
  &\red (\lambda x. x \langle a \rangle) \langle b \rangle \\
  &\red b \langle a \rangle.
\end{align*}
Hence we should not use this calculus as a representation of plays: it seems quite hard to prove the associativity of composition.
}

\tk{NOTE: I remove indexes from the terms.  The indexes are implicitly controlled by the syntax.  That means, for \( \lambda \bar{x}. ({\sf p}_i x)\,A_1\,\dots\,A_n \), it must be the case that \( i \) is less than indexes for \( x \) in \( A_1, \dots, A_n \).  Furthermore we require, for every variable \( x \), indexes appearing in \( A_k \) must be less than those in \( A_{k+1} \). In this way, the index for each occurrence is uniquely determined (provided that the set of indexes is a subset of natural numbers of the form \( [1;N] \) for some \( N \)).} \lo{If the requirement is that each occurrence is uniquely determined, then the (implicit) indices should presumably start from 1 i.e.~the leftmost occurrence should have index 1. If so, then the set of indices of a variable in a term is always $[1;m]$ for some $m$. Am I right?}  \tk{Right.}
\tk{By this representation, one can easily establish the connection between plays and terms.  Another option is to change the representation of plays to fit the indexed-term representation by introducing the notion of indexes to plays (so that each occurrence of moves has its index). Then the composition of plays should be defined using these indexes instead of the sequential structure of plays.  I did not choose this since the definition of plays and their composition (perhaps) look very different from the standard definitions.  This representation of plays resembles \cite{DiGianantonioL13} (although they did not characterise the well-formed partitioned positions (NEED TO CHECK), which correspond to the plays).}

This notion corresponds to the notion of plays (but not exactly the same).  Hence it can be represented by terms in normal form (recall the connection between plays and B\"ohm trees, which is a kind of normal form).

The calculus is essentially the same as the \emph{non-uniform \( \lambda \)-calculus} of Melli\'es~\cite{Mellies2006} \tk{But our calculus is finite and linear.} and \emph{multilinear-visible representation of a (poly-)term} by Ehrhard and Regnier~\cite{Ehrhard2008}.  % \lo{@Takeshi: I can't find the phrase ``multilinear-free representation'' in \cite{Ehrhard2008}. Do you mean ``multilinear-visible''?} \tk{@Luke: Right.  What I referred is the HAL version (i.e. a draft version), in which this notion is called ``multilinear-free representation''.  Thanks.}
\tk{We should mention the work \cite{Mazza12}.}
\emph{Terms} and \emph{lists} are defined by

The calculus is essentially the same as the \emph{non-uniform \( \lambda \)-calculus} of Melli\'es~\cite{Mellies2006} \tk{But our calculus is finite and linear.} and \emph{multilinear-free \lo{multilinear-visible(?)} representation of a (poly-)term} by Ehrhard and Regnier~\cite{Ehrhard2008}.  \lo{@Takeshi: I can't find the phrase ``multilinear-free representation'' in \cite{Ehrhard2008}. Do you mean ``multilinear-visible''?} \tk{@Luke: Right.  What I referred is the HAL version (i.e. a draft version), in which this notion is called ``multilinear-free representation''.  Thanks.} \tk{We should mention the work \cite{Mazza12}.}
\emph{Linear terms} are defined by
\[
\begin{array}{lrlcl}
  \textit{Term}&(\Lambda^{\wedge}_{\nf})\quad&
  M, N &{}::={}& \lambda \bar{x}. y\,T_1\,\dots\,T_k
  \\
  \textit{List}&(\bar{\Lambda}^{\wedge}_{\nf})\quad&
  T, U &{}::={}& \langle M_1, \dots, M_n \rangle \textrm{\qquad(\( n \ge 0 \))}.
\end{array}
\]


The \emph{approximation order} of terms are defined by the following rules.  We are interested in how a term can be embedded into another term.  For example, we distinguish two embedding from \( \langle \lambda x. x\,\langle \rangle\;\rangle \) into \( \langle \lambda y. y \langle e_1, e_2 \rangle,\, \lambda z. z \langle h_1, h_2, h_3 \rangle\;\rangle \), identifying \( x \) with \( y \) and \( z \), respectively.  So we define the approximation relation as a triple, \( \varphi \rhd A \sqsubseteq B \), where \( A \) and \( B \) are terms and \( \varphi \) is a witness describing how to embed.
%
\infrule{
  \forall k \in [1;n].\ T_k \sqsubseteq U_k
}{
  (\lambda \bar{x}. y\,T_1\,\dots\,T_n) \sqsubseteq (\lambda \bar{x}. y\,U_1\,\dots\,U_n)
}
\infrule{
  \exists \vartheta : [1;n] \stackrel{\textrm{injection}}{\longrightarrow} [1;m]
  \qquad
  \forall i \in [1;n].\ M_i \sqsubseteq N_{\vartheta(i)}
}{
  \langle M_1, \dots, M_n \rangle \sqsubseteq \langle N_1, \dots, N_m \rangle
}
%

We are interested not only in whether a term can be embedded into another term, but also in how we can embed and how many way.  This is in parallel to the game semantic category of plays, in which we distinguish the way to embed.  \tk{For example, \( \langle \lam x. x \langle \rangle \rangle \) can be embedded into \( \langle \lam x.x \langle \rangle, \lam x. x \langle x \rangle \rangle \) in two ways.}

A way to achieve this is to introduce a term representation of the above rules.  However we adopt a different approach based on an intersection type system.  This type system will be used for another purpose.

\paragraph{Intersection type assignment}
The syntax of types are given by:
\[
\begin{array}{llcl}
  (\textit{Prime type})\quad&
  A, B &{}::={}& \T \mid A^! \multimap B
  \\
  (\textit{Intersection type})\quad&
  A^!, B^! &{}::={}& A_1 \wedge \dots \wedge A_n
\end{array}
\]
where \( n \ge 0 \).  We write \( \tensorunit \) for the empty intersection.  The intersection of intersection types is defined by:
\[
  (A_1 \!\wedge\! \dots \!\wedge\! A_n) \wedge (B_1 \!\wedge\! \dots \!\wedge\! B_m)
  := A_1 \!\wedge\! \dots \!\wedge\! A_n \!\wedge\! B_1 \!\wedge\! \dots \!\wedge\! B_m.
\]
The intersection is assume to be associative, but not commutative (i.e.~\( A \wedge B \neq B \wedge A \)) nor idempotent (i.e.~\( A \wedge A \neq A \)).  However \( A \wedge B \) is isomorphic to \( B \wedge A \) in a certain sense and this isomorphism plays an important role.  \tk{This isomorphism corresponds to reindexing.  It might be better to point out this and the connection to AJM games or Melli{\'e}s's orbital games.}  We use the metavariables like \( A^! \) and \( B^! \) for intersection types, because the intersection types are finite exponential-free approximations of the exponentials.

The intersection is very closed to the tensor of linear logic \tk{Should I cite something?}, but the intersection does not satisfy the law \( A \wedge B \multimap C \eqty A \multimap B \multimap C \).

A \emph{type environment} is a finite partial function from variables to intersection types, represented by a finite sequence.  The typing rules are listed as follows.
%
\infrule{
  \mathstrut
}{
  x : A \vdash x : A
}
\infrule{
  \Gamma_1 \vdash M : A^! \multimap B
  \qquad
  \Gamma_2 \vdash T : A^!
}{
  \Gamma_1 \wedge \Gamma_2 \vdash M\,T : B
}
\infrule{
  \Gamma, x : A^! \vdash M : B
}{
  \Gamma \vdash M : A^! \multimap B
}
\infrule{
  \forall i \in [1;n].\ \Gamma_i \vdash M_i : A_i
}{
  \Gamma_1 \wedge \dots \wedge \Gamma_n \vdash \langle M_1, \dots, M_n \rangle : A_1 \wedge \dots \wedge A_n
}
%
In the last rule, the tensor of type environments is defined by point-wise tensor.  A derivation is \emph{\( \eta \)-long} if every applications are fully-applied.

\begin{lemma}
Every term \( M \) has a unique \( \eta \)-long derivation.  Hence the map \( M \mapsto (\Gamma \vdash A) \), where \( \Gamma \vdash M : A \) has a \( \eta \)-long derivation, is a well-defined function.
\end{lemma}
\begin{proof}
By induction on the structure of \( M \).  The \( \eta \)-long condition is used to determine the type for variables.
\tk{The relaxed version of this lemma holds for general terms.  The relaxed version ensures only uniqueness of \( \eta \)-long derivation, but not the existence.}
\end{proof}

This lemma encourages us to study the normal terms via types.  As we shall see, this is essentially the GoI interpretation. \tk{Need justification?}

\tk{TODO: some words}
%
\infrule{
  \mathstrut
}{
  \BM \rhd \T \subty \T
}
\infrule{
  \varphi \rhd A^!_1 \subty B^!_1
  \qquad
  \vartheta \rhd A_2 \subty B_2
}{
  (\varphi \multimap \vartheta) \rhd (A^!_1 \multimap A_2) \subty (B^!_1 \multimap B_2)
}
\infrule{
  \varphi : [1;n] \stackrel{\mathrm{injection}}{\longrightarrow} [1;m]
  \qquad
  \forall i \in [1;n].\ \vartheta_i \rhd A_i \subty B_{\varphi(i)}
}{
  (\bigwedge_{i \in [1;n]}^{\varphi} \vartheta_i) \rhd (A_1 \wedge \dots \wedge A_n) \subty (B_1 \wedge \dots \wedge B_m)
}
%
Let \( \Phi \) be a partial map from variables to witnesses.  We write \( \Phi \rhd \Gamma \subty \Gamma' \) if \( \dom(\Phi) = \dom(\Gamma) \) and \( \Phi(x) \rhd \Gamma(x) \subty \Gamma'(x) \) for every \( x \in \dom(\Gamma) \).  We write \( (\Phi \vdash \varphi) \rhd (\Gamma \vdash A) \subty (\Gamma' \vdash A') \) if \( \Phi \rhd \Gamma \vdash \Gamma' \) and \( \varphi \rhd A \subty A' \).

Let \( \Gamma \vdash M : A \) and \( \Gamma' \vdash M' : A' \) and \( (\Phi \vdash \varphi) \rhd (\Gamma \vdash A) \subty (\Gamma' \vdash A') \).  The relation \( (\Phi \vdash \varphi) \rhd (\Gamma \vdash M : A) \sqsubseteq (\Gamma' \vdash M' : A') \) is defined by induction on derivations:
%
\infrule{
  (\Phi[x \mapsto \psi], \varphi) \rhd (\Gamma, x : \vec{A} \vdash M : B) \sqsubseteq (\Gamma', x : \vec{A}' \vdash M' : B')
}{
  (\Phi, (\psi, \varphi)) \rhd (\Gamma \vdash \lam x. M : \vec{A} \multimap B) \sqsubseteq (\Gamma' \vdash \lam x. M' : \vec{A}' \multimap B')
}
\infrule{
  \exists \vartheta \rhd \vec{B} \subty \vec{B}' \\
  (\Phi_1, (\vartheta, \varphi)) \rhd (\Gamma_1 \vdash M : \vec{B} \multimap A) \sqsubseteq (\Gamma'_1 \vdash M' : \vec{B}' \multimap A')
  \\
  (\Phi_2, \vartheta) \rhd (\Gamma_2 \vdash T : \vec{B}) \sqsubseteq (\Gamma'_2 \vdash T' : \vec{B}')
}{
  (\Phi_1 \wedge \Phi_2, \varphi) \rhd (\Gamma_1 \wedge \Gamma_2 \vdash M\,T : A) \sqsubseteq (\Gamma'_1 \wedge \Gamma'_2 \vdash M'\,T' : A')
}
\infrule{
  \forall i \in [n].\ (\Phi_i, \varphi_i) \rhd (\Gamma_i \vdash M_i : A_i) \sqsubseteq (\Gamma'_{\vartheta(i)} \vdash M'_{\vartheta(i)} : A'_{\vartheta(i)})
}{
  (\bigwedge_{i \in [n]} \Phi_i, (\vartheta, (\varphi_i)_{i \in [n]})) \\
  \rhd (\bigwedge_{i \in [n]} \Gamma_i \vdash \langle M_i \rangle_{i \in [n]} : \bigwedge_{i \in [n]} A_i) \sqsubseteq (\bigwedge_{j \in [m]} \Gamma'_j \vdash \langle M'_j \rangle_{j = [m]} : \bigwedge_{j = [m]} A'_j)
}
%
\tk{What is the point?}  \tk{Games are based on the sequential structure with justification.  Types are based on the justification structure and sequential structure is captured by the above rules.}

The composition is defined by: \( \BM \circ \BM := \BM \), \( (\varphi' \multimap \vartheta') \circ (\varphi \multimap \vartheta) := (\varphi' \circ \varphi) \multimap (\vartheta' \circ \vartheta) \) and
\[
  (\bigwedge_{j \in [m]}^{\varphi'} \vartheta'_j) \circ (\bigwedge_{i \in [n]}^{\varphi} \vartheta_i) := \bigwedge_{i \in [n]}^{\varphi' \circ \varphi} \vartheta'_{\varphi(i)} \circ \vartheta_i.
\]
The composition can be straightforwardly extended to \( \Phi \rhd \Gamma \subty \Gamma' \) and \( (\Phi \vdash \varphi) \).
\begin{lemma}
Suppose that 
\[
  (\Gamma_1 \vdash M_1 : A_1) \stackrel{\Phi \vdash \varphi}{\longrightarrow}
  (\Gamma_2 \vdash M_2 : A_2) \stackrel{\Phi' \vdash \varphi'}{\longrightarrow}
  (\Gamma_3 \vdash M_3 : A_3).
\]
Then \( (\Phi' \vdash \varphi') \circ (\Phi \vdash \varphi) : (\Gamma_1 \vdash M_1 : A_1) \to (\Gamma_3 \vdash M_3 : A_3) \).
\end{lemma}

Hence they form a category.  \tk{state associativity of the composition.  Existence of the identity is rather trivial.}

For a function \( f : A \to B \), its image is defined by \( \codom(f) := \{ f(a) \mid a \in A \} \).  Let us fix a kind \( \kappa \) and consider the category \( \mathbbm{B}_{\kappa} \).  Assume an object \( e \in \mathbbm{B}_{\kappa} \) and a family of maps \( \{ \varphi^\xi : e^{\xi} \to e \}_{\xi \in \Xi} \).  This family \emph{covers} \( e \) just if the union of the image of \( \varphi_\xi \), as $\xi$ ranges over $\Xi$, is \( e \).  This notion can be formally defined by induction on \( e \):
\begin{itemize}
\item If \( e = \lambda \bar{x}. y\,A_1\,\dots\,A_n \), then for each \( \xi \in \Xi \), we have \( e^{\xi} = \lambda \bar{x}. y\,A^{\xi}_1\,\dots\,A^{\xi}_n \) and \( \varphi^\xi = (\varphi^\xi_1, \dots, \varphi^\xi_n) \).  The family covers \( e \) just if
  \begin{enumerate}
  \item The family is nonempty, and
  \item \( \{ \varphi^{\xi}_k : A^{\xi}_k \to A_k \}_{\xi \in \Xi} \) covers \( A_k \) for every \( k \).
  \end{enumerate}
\end{itemize}
For lists, we define
\begin{itemize}
\item For a list \( A = \langle e_1, \dots, e_n \rangle \), consider the family \( \{ \varphi^{\xi} : A^{\xi} \to A \}_{\xi \in \Xi} \).  We have \( A^{\xi} = \langle e^{\xi}_1, \dots, e^{\xi}_{n^{\xi}} \rangle \) and \( \varphi^{\xi} = (\vartheta^{\xi}, (\varphi^{\xi}_j)_{j \in [1; n^{\xi}]}) \).  This family covers \( A \) just if, for every \( i \in [1;n] \), the family \( \{ \varphi^{\xi}_j : e^{\xi}_j \to e_i \mid \vartheta^{\xi}(j) = i \} \) covers \( e_i \).
\end{itemize}
Notice that this condition implies that \( [1;n] = \bigcup_{\xi \in \Xi} \codom(\vartheta^{\xi}) \).  Otherwise, for \( i \in I - (\bigcup_{\xi \in \Xi} \codom(\vartheta^{\xi}) \), the family \( \{ \varphi^{\xi}_j : e^{\xi}_j \to e_i \mid \vartheta^{\xi}(j) = i \} \) is empty and thus cannot cover \( e_i \).

\tk{TODO: terminology}


\tk{We introduce a simple-type assignment system for normal terms.  The typing rules are listed as follows.}
%
\infrule{
  y :: \delta_1 \to \dots \to \delta_m \to \T \in \Gamma \hfill
  \\
  \forall k \in [1;m].\quad \Gamma, x_1 :: \kappa_1, \dots, x_n :: \kappa_n \vdash A_k :: \delta_k
}{
  \Gamma \vdash \lambda x_1 \dots x_n. y\,A_1\,\dots\,A_m :: \kappa_1 \to \dots \to \kappa_n \to \T
}
\infrule{
  \forall k \in [1;n].\ \Gamma \vdash e_i :: \kappa
}{
  \Gamma \vdash \langle e_1, \dots, e_n \rangle :: \kappa
}
%

\begin{definition}
\tk{Define a category \( \mathbb{B}_{\Gamma, \Delta} \).}  \tk{\( \mathbb{B}_{\kappa} \) is a full subcategory.}
\end{definition}




\subsection{Adjoint equivalence}
We have defined the category of plays \( \mathbb{P}_A \) for an arena \( A \) and the category of terms \( \mathbb{B}_\kappa \) for a kind \( \kappa \).  This subsection establishes an equivalence between \( \mathbb{P}_{\kappa} \) and \( \mathbb{B}_{\kappa} \), where \( \mathbb{P}_{\kappa} \) is the category of plays of the arena corresponding to \( \kappa \).

\subsubsection{From kinds to arenas}
Given a kind \( \kappa \), the set of \emph{paths} \( \mathit{Path}(\kappa) \subseteq \Nat^* \) is a (finite) set defined by:
\(
  \mathit{Path}(\kappa_1 \to \dots \to \kappa_n \to \T) := \{ \varepsilon \} \cup \{ k \, \pi \mid k \in [1;n], \pi \in \mathit{Path}(\kappa_k) \}
\).
The arena \( A(\kappa) \) is defined as \( (\mathit{Path}(\kappa), \lambda, \vdash) \) where
\begin{itemize}
\item \( \lambda(\pi) := \OO \) if the length of \( \pi \) is odd, and
\item \( \pi \vdash \pi' \) when \( \pi' = k \, \pi \) for some \( k \in \Nat \), \( \star \vdash \pi \) when \( \pi = \varepsilon \).
\end{itemize}

\subsubsection{From terms to plays}
We use an alternative representation of plays in which O-moves has pointers and P-moves does not have pointers but have variable name.  So in a sequence the pointer from a P-move labelled \( x \) is the abstraction that introduces the name \( x \), i.e.~a move of the form \( \lambda \bar{y} \) where \( x \in \bar{y} \).
\begin{align*}
  F(\lambda \bar{x}. y\,T_1\,\dots\,T_n) &:= [\lambda \to \T] \bar{x}]\;[y]\; F(T_1)\;\dots\;F(T_n) \\
  F(\langle M_1, \dots, M_n \rangle) &:= F(M_1) \dots F(M_n)
\end{align*}
where in the first expression the initial moves of \( F(T_i) \) points to \( [y] \).  The justification pointer is defined as described above.  The map to a move label is the type for each node, i.e.~\( [\lambda \bar{x}] \mapsto \bar{\kappa} \to \T \) (where \( \bar{\kappa} = \kappa_1 \to \dots \to \kappa_n \) is the sequence of simple types of the variables \( \bar{x} = x_1 x_2 \dots x_n \)) and \( [y] \mapsto \kappa \) (where \( \kappa \) is the simple type for \( y \)).

\tk{Define the morphism part.}

\begin{lemma}
\( F \) is a functor.
\end{lemma}

\subsubsection{From plays to terms}
\tk{TODO: define \( G \).}

\lochanged{We define a functor $G : \cat{P}_\kappa \to \cat{B}_\kappa$ as follows. First the map on objects. In the base case, $G$ maps the empty play to $\anglebra{}$. For the inductive case, take a play $s \, m_1^O \, m_2^P$. Suppose $m^O_1$ is initial, then it follows from P-visibility that $m_2^P$ is justified by $m_1^O$, and so, $G(s \, m_1^O \, m_2^P) := \anglebra{e_1, \ldots, e_n, \lambda \bar{x}.x_i}$ where $G(s) = \anglebra{e_1, \ldots, e_n}$ and $m_2^P$ is the $i$-child of $m_1^O$. Now suppose $m_1^O$ is justified by the move $m_0^P$, which occurs in $s$. By O-justification, we may assume that $G(s) = C[x \, A_1 \ldots A_i \ldots A_m]$ where $C[\,]$ is a term context, $[x] = m_0^P$ (i.e.~$x$ corresponds to $m_0^P$), $m_1^O$ is the $i$-child of $m_0^P$, and $A_i = \anglebra{e_1, \ldots, e_n}$. Then $G(s \, m_1^O \, m_2^P) := C[x \, A_1 \ldots \anglebra{e_1, \ldots, e_n, \lambda \bar{x}.y} \ldots A_m]$ where $[\lambda \bar{x}] = m_1^O$ and $[y] = m_2^P$.}

\lo{Ongoing}

\begin{lemma}
The pair of functors \( F \) and \( G \) forms an adjoint equivalence.  They preserve and reflect the covering families.  \tk{TODO: check the correctness of the terminology.}
\end{lemma}





\subsection{Interaction of normal \( \lambda^{\wedge} \)-terms}
Basically the interaction between terms \( M \) and \( N \) is just their application \( M\,N \).  Three projections are the projection to the function \( M\,N \mapsto M \), the projection to the argument \( M\,N \mapsto N \) and the \emph{normalisation} mapping \( M\,N \) to its normal form.

So we have two things to define, the normalisation process and the approximation relation for applications.

In order to define normalisation, we first define substitution.  Given a term \( M \), a variable \( x \) and a list \( U \), we write \( \Subst{M}{x \mapsto U}{M'} \) for the substitution of the free occurrences of \( x \) in \( M \) by elements of \( U \).  Where the left-most occurrence of \( x \) is replaced with the left-most element in \( U \) and the second with the second, and so on.  Formally the substitution is defined by the following rules.
%
\infrule{
  \mathstrut
}{
  \Subst{x}{x \mapsto \langle M \rangle}{M}
}
\infrule{
  \mathstrut
}{
  \Subst{y}{x \mapsto \langle\;\rangle}{y}
}
\infrule{
  \Subst{M}{x \mapsto T}{M'}
}{
  \Subst{(\lambda y. M)}{x \mapsto T}{\lambda y. M'}
}
\infrule{
  \Subst{M}{x \mapsto T_1}{M'}
  \qquad
  \Subst{U}{x \mapsto T_2}{U'}
}{
  \Subst{(M\,U)}{x \mapsto (T_1; T_2)}{M'\,U'}
}
\infrule{
  \forall i \in [1;n].\ \Subst{M_i}{x \mapsto T_i}{M'_i}
}{
  \Subst{(\langle M_1, \dots, M_n \rangle)}{x \mapsto (T_1; \dots; T_n)}{\langle M'_1, \dots, M'_n \rangle}
}
%
Here \( (T_1; T_2) \) is the concatenation, e.g.
\[
  \langle M_1, \dots, M_m \rangle; \langle N_1, \dots, N_n \rangle = \langle M_1, \dots, M_m, N_1, \dots, N_n \rangle.
\]
Notice that the substitution is well-defined only if the length of the list is equivalent to the number of occurrences of \( x \) in \( M \).

Reduction (head reduction): \( E ::= \square \mid \lam x. E \mid x\,T_1\,\dots\,T_{i-1}\,E\,T_{i+1}\,\dots\,T_n \mid \langle M_1, \dots, M_{i-1}, E\, M_{i+1}, \dots, M_n \rangle \).
%
\infrule{
  \Subst{M}{x \mapsto T}{M'}
}{
  (\lambda x. M)\,T \red e'
}
\infrule{
  M \red M'
}{
  E[M] \red E[M']
}
%% \infrule{
%%   M \red M'
%% }{
%%   \lam x. M \red \lam x. M'
%% }
%% \infrule{
%%   M_i \red M'_i
%% }{
%%   \langle M_1, \dots, M_n \rangle \red
%%   \langle M_1, \dots, M_{i-1}, M'_i, M_{i+1}, \dots, M_n \rangle
%% }
%% \infrule{
%%   T_i \red T'_i
%% }{
%%   x\,T_1\,\dots\,T_n \red x\,T_1\,\dots\,T_{i-1}\,T'_i\,T_{i+1}\,\dots\,T_n
%% }
%
This reduction strategy is nothing but the left-most reduction strategy where the priority of the completely independent redex is not fully determined (see the last rule).

We write \( \normalise{s}{t} \) when \( s \red^* t \) and \( t \) is a normal form.

However the normalisation process of \( \lambda^{\wedge} \) is not as good as that of simply-typed \( \lam \)-calculus.  First the normalisation process of \( \lambda^{\wedge} \) may get stuck, for instance, consider the term \( (\lam x. x) \langle M, M \rangle \), in which the list has more elements than required.  We shall introduce a type system as in \cite{Kfoury2000} that removes badly behaved terms.  Second since the reduction changes the left-to-right order of occurrences of variables, as in
\[
  (\lam x. x\,\langle y_1 \rangle) \langle y_2 \rangle \red y_2\,\langle y_1 \rangle
\]
(where \( y_1 \) and \( y_2 \) are different occurrences of the same variable \( y \)),  the full reduction is not confluent.  For instance,
\[
  (\lam y. (\lam x. x\,\langle y \rangle)\,\langle y \rangle)\,\langle a, b \rangle \red (\lam x. x\,\langle a \rangle)\,\langle b \rangle \red b\,\langle a \rangle
\]
when we follow the strategy we adopted (i.e.~the left-most strategy), but
\[
  (\lam y. (\lam x. x\,\langle y \rangle)\,\langle y \rangle)\,\langle a, b \rangle \red (\lam y. y\,\langle y \rangle)\,\langle a, b \rangle \red a\,\langle b \rangle
\]
when we reduce the inner redex first (though it is prohibited by the strategy).  The same problem causes the failure of the type preservation.\footnote{Kfoury has shown that the type preservation and confluence of \( \lambda^{\wedge} \) in his paper~\cite{Kfoury2000}, but the proofs have errors.  \tk{TODO: check}}

\begin{remark}
This problem has been addressed by some work.  For example, this is the reason why AJM game model uses an equivalence class of strategies instead of strategies.  The failure of the type preservation can be found in several ``rigid'' intersection type systems such as (POPL intersection type inference, ICFP 2006, Game types).  So the way to handle this problem is not trivial and not uninterested.  \tk{TODO: check the paper assigning linear types for cbv terms.}
\end{remark}

\paragraph{IMLL type assignment}
We use formulas of the intuitionistic multiplicative linear logic (IMLL) for removing badly behaved terms.  The syntax of types are given by:
\[
\begin{array}{llcl}
  (\textit{Prime type})\quad&
  A, B &{}::={}& \T \mid A^! \multimap B
  \\
  (\textit{Intersection type})\quad&
  A^!, B^! &{}::={}& A_1 \wedge \dots \wedge A_n
\end{array}
\]
where \( n \ge 0 \).  We write \( \tensorunit \) for the empty intersection.  The intersection of intersection types is defined by:
\[
  (A_1 \!\wedge\! \dots \!\wedge\! A_n) \wedge (B_1 \!\wedge\! \dots \!\wedge\! B_m)
  := A_1 \!\wedge\! \dots \!\wedge\! A_n \!\wedge\! B_1 \!\wedge\! \dots \!\wedge\! B_m.
\]
The intersection is assume to be associative, but not commutative (i.e.~\( A \wedge B \neq B \wedge A \)) nor idempotent (i.e.~\( A \wedge A \neq A \)).  However \( A \wedge B \) is isomorphic to \( B \wedge A \) in a certain sense and this isomorphism plays an important role.  \tk{This isomorphism corresponds to reindexing.  It might be better to point out this and the connection to AJM games or Melli{\'e}s's orbital games.}  We use the metavariables like \( A^! \) and \( B^! \) for tensor types, because the intersection types are finite exponential-free approximations of the exponentials.

The intersection is very closed to the tensor of linear logic \tk{Should I cite something?}, but the intersection does not satisfy the law \( A \wedge B \multimap C \eqty A \multimap B \multimap C \).

A \emph{type environment} is a finite partial function from variables to tensor types, represented by a finite sequence.  The typing rules are listed as follows.
%
\infrule{
  \mathstrut
%  \textrm{\tk{Perhaps we need to allow applying iso.}}  \textrm{\tk{We do not need, since we do not handle index permutations.}}
}{
  x : A \vdash x : A
}
\infrule{
  \Gamma_1 \vdash M : A^! \multimap B
  \qquad
  \Gamma_2 \vdash T : A^!
}{
  \Gamma_1 \wedge \Gamma_2 \vdash M\,T : B
}
\infrule{
  \Gamma, x : A^! \vdash M : B
}{
  \Gamma \vdash M : A^! \multimap B
}
\infrule{
  \forall i \in [1;n].\ \Gamma_i \vdash M_i : A_i
}{
  \Gamma_1 \otimes \dots \otimes \Gamma_n \vdash \langle M_1, \dots, M_n \rangle : A_1 \otimes \dots \otimes A_n
}
%
In the last rule, the tensor of type environments is defined by point-wise tensor.

A tensor type binding \( x : A_1 \otimes \dots \otimes A_n \) in an environment expresses that the variable \( x \) has \( n \) occurrences in the subject term.  The order of \( A_i \)s in the tensor corresponds to the left-to-right order of occurrences of \( x \) in the term, e.g.~\( A_1 \) is the type for the left-most occurrence of \( x \) and \( A_2 \) is for the next.

Hence the reduction does not preserve types: setting \( M = (\lam x. x\,\langle y \rangle)\,\langle y \rangle \), we have \( y : \T \otimes (\T \multimap \T) \vdash M : \T \) and \( M \red y\,\langle y \rangle \), but not \( y : \T \otimes (\T \multimap \T) \vdash y\,\langle y \rangle : \T \).  This happens because the reduction may change the left-to-right ordering of variables, e.g.~the left occurrence of \( y \) in \( M \) corresponds to the right occurrence in \( y\,\langle y \rangle \).  However the judgement is easily corrected by permuting the tensor type in the environment: \( y : (\T \multimap \T) \otimes \T \vdash y\,\langle y \rangle : \T \).  We shall develop a precise handling of this phenomenon.

We say \( M \) is typable if \( \Gamma \vdash M : A \) for some \( \Gamma \) and \( A \).  \emph{Interleaving} of two intersection types, written \( \vec{A} \parallel \vec{B} \) is a set of intersection types defined by: \( \vec{A} \parallel \tensorunit := \{ \vec{A} \} \) and \( \tensorunit \parallel \vec{B} := \{ \vec{B} \} \) and
\begin{align*}
  (A \wedge \vec{A}) \parallel (B \wedge \vec{B}) :=&\; \{ A \wedge \vec{C} \mid \vec{C} \in (\vec{A} \parallel (B \wedge \vec{B})) \} \\
  \cup &\; \{ B \wedge \vec{C} \mid \vec{C} \in ((A \wedge \vec{A}) \parallel \vec{B}) \}.
\end{align*}
We write \( \Delta \in (\Gamma \parallel \Gamma') \) if \( \Delta(x) \in (\Gamma(x) \parallel \Gamma'(x)) \) for every \( x \).
\begin{lemma}[Substitution]\label{lem:vec-substitution}
Let \( \Gamma, x : \vec{A} \vdash M : B \) and \( \Gamma' \vdash T : \vec{A} \).  Then \( \Subst{M}{x \mapsto T}{M'} \) for some \( M' \).  Furthermore \( \Delta \vdash M' : B \) with \( \Delta \in (\Gamma \parallel \Gamma') \).  The same statement holds for vectors.
\end{lemma}
\begin{proof}
By induction on the structure of \( M \) (terms) and \( U \) (vectors).
\begin{itemize}
\item Case \( M = x \): Then \( \Gamma = \emptyset \) and \( \vec{A} = B \).  We have \( \Gamma' \vdash T : B \), which implies \( T = \langle N \rangle \) and \( \Gamma' \vdash N : B \).  By definition, we have \( \Subst{x}{x \mapsto \langle N \rangle}{N} \) as desired.
\item Case \( M = y \): Then \( \Gamma = y : B \) and \( \vec{A} = \mathbf{1} \).  We have \( \Gamma' \vdash T : \mathbf{1} \), which implies \( T = \langle\;\rangle \) and \( \Gamma' = \emptyset \).  We have \( \Subst{y}{x \mapsto \langle\;\rangle}{y} \) as desired.
\item Case \( M = \lambda y. M_0 \): Then \( B = \vec{B}_0 \multimap B_1 \) and \( \Gamma, y : \vec{B}_0, x : \vec{A} \vdash M_0 : B_1 \).  By the induction hypothesis, \( \Subst{M_0}{x \mapsto T}{M'_0} \) for some \( M'_0 \) and thus \( \Subst{(\lambda y. M_0)}{x \mapsto T}{\lambda y. M'_0} \).  By the induction hypothesis, we have \( \Delta, y : \vec{B}'_0 \vdash M_0 : B_1 \), where \( (\Delta, y : \vec{B}'_0) \in ((\Gamma, y : \vec{B}_0) \parallel \Gamma') \).  Since \( y \) is not in the domain of \( \Gamma' \) (i.e.~\( \Gamma'(y) = \mathbf{1} \)), we know that \( \vec{B}'_0 = \vec{B}_0 \).  By applying the abstraction rule, we have \( \Delta \vdash \lambda y. M_0 : \vec{B}_0 \multimap B_1 \).  It is easy to check that \( \Delta \in (\Gamma \parallel \Gamma') \).
\item Case \( M = M_0\,U \): Then we have \( \Gamma_0, x : \vec{A}_0 \vdash M_0 : \vec{C} \multimap B \) and \( \Gamma_1, x : \vec{A}_1 \vdash U : \vec{C} \) with \( \Gamma = \Gamma_0 \wedge \Gamma_1 \) and \( \vec{A} = \vec{A}_0 \wedge \vec{A}_1 \).  Since \( \Gamma' \vdash T : \vec{A}_0 \wedge \vec{A}_1 \), we have \( \Gamma'_0 \vdash T_0 : \vec{A}_0 \) and \( \Gamma'_1 \vdash T_1 : \vec{A}_1 \) with \( T = (T_0;T_1) \) and \( \Gamma' = \Gamma'_0 \wedge \Gamma'_1 \).  By the induction hypothesis, we have \( \Subst{M_0}{x \mapsto T_0}{M_0'} \) and \( \Subst{U}{x \mapsto T_1}{U'} \) and \( \Delta_0 \vdash M'_0 : \vec{C} \multimap B \) and \( \Delta_1 \vdash U' : \vec{C} \) with \( \Delta_0 \in (\Gamma_0 \parallel \Gamma'_0) \) and \( \Delta_1 \in (\Gamma_1 \parallel \Gamma'_1) \).  Hence we have \( \Delta_0 \wedge \Delta_1 \vdash M_0\,U : B \).  It is easy to check that \( \Delta_0 \wedge \Delta_1 \in ((\Gamma_0 \wedge \Gamma_1) \parallel (\Gamma'_0 \wedge \Gamma'_1)) \).
\end{itemize}
It is easy to prove the case for vectors.
\end{proof}

\begin{lemma}[Preservation of typability]
Let \( M \) be a typable term.  If \( M \red M' \), then \( M' \) is typable.
\end{lemma}
\begin{proof}
Assume that \( \Gamma \vdash M : A \).  We prove the claim by induction on the derivation of \( M \red M' \).  The only nontrivial case is \( (\lambda x. M)\,T \red M' \) where \( \Subst{M}{x \mapsto T}{M'} \).  This case is a consequence of Lemma~\ref{lem:vec-substitution}.
\end{proof}

\begin{lemma}
Assume \( \Gamma \vdash M : A \) and \( M \red M' \).  Then \( \Gamma' \vdash M : A' \) and \( (\Phi, \varphi) \rhd (\Gamma \vdash A) \peqty (\Gamma' \vdash A') \) for some \( \Gamma' \), \( A' \), \( \Phi \) and \( \varphi \).
\end{lemma}

\begin{lemma}
Assume that \( \Gamma \vdash U : A^! \) and \( (\Phi, \varphi) \rhd (\Gamma \vdash A^!) \oeqty (\Delta \vdash B^!) \).  Then there uniquely exists \( V \) such that \( \vartheta_{\Phi, \varphi} \rhd U \approx V \).  Furthermore \( \Delta \vdash V : B^! \).  A similar statement holds for terms.
\end{lemma}
\begin{proof}
By induction on the structure of terms.  Assume that \( \Gamma \vdash U : A_1 \otimes \dots \otimes A_n \).  Then \( \Gamma = \Gamma_1 \otimes \dots \otimes \Gamma_n \) and \( U = \langle M_1, \dots, M_n \rangle \) with \( \Gamma_i \vdash M_i : A_i \) for every \( i \).  Suppose that \( \varphi = (\varphi_0, (\varphi_i)_{i \in [1;n]}) \).  Then \( B^! = B_1 \otimes \dots \otimes B_n \) and \( \varphi_i \rhd A_i \oeqty B_{\varphi_0(i)} \) for every \( i \in [1;n] \).  Since \( \Phi \rhd (\Gamma_1 \otimes \dots \otimes \Gamma_n) \peqty \Delta \), we know that \( \Phi \) acts as identity on the top-level tensor and thus we can decompose \( \Delta \) as \( (\Delta_i)_{i \in [1;n]} \) with \( \Phi_i \rhd \Gamma_i \peqty \Delta_i \) for all \( i \) (and these morphisms suffice to recover \( \Phi \)).  By the induction hypothesis, for each \( i \in [1;n] \), we have a unique \( N_i \) such that \( \vartheta_{\Phi_i, \varphi_i} \rhd M_i \approx N_i \) and \( \Delta_i \vdash N_i : B_i \).
\end{proof}

\paragraph{Embedding of terms}
If \( M \) is in normal form (i.e.~in \( \eta \)-long \( \beta \)-normal form), the type judgement for \( M \) is uniquely determined.  \tk{Here we need to restrict the refinements of types.}
\begin{lemma}
Let \( \Delta \vdash M :: \kappa \) be a simply-typed term in normal form.  Then there exists unique \( \Gamma :: \Delta \) and \( A :: \kappa \) such that \( \Gamma \vdash M : A \).
\end{lemma}
\begin{proof}
By induction on the structure of \( M \).  The case in which \( M = \lam x. M_0 \) is easy.  Assume that \( M = x\,T_1\,\dots\,T_n \).  Since \( M \) is in \( \eta \)-long form, the simple type for \( x \) is \( \delta_1 \to \dots \to \delta_n \to \T \) and hence the type for \( x \) must be of the form \( A_1 \multimap \dots \multimap A_n \multimap \T \) because it is a refinement of the simple type.  So the type for \( x \) is uniquely determined by types for \( T_i \)'s.  Hence we have the claim.
\end{proof}

%
\infrule{
  \mathstrut
}{
  () \rhd \T \subty \T
}
\infrule{
  \varphi \rhd A^!_1 \subty B^!_1
  \qquad
  \vartheta \rhd A_2 \subty B_2
}{
  (\varphi, \vartheta) \rhd (A^!_1 \multimap A_2) \subty (B^!_1 \multimap B_2)
}
\infrule{
  \varphi : [1;n] \stackrel{\mathrm{injection}}{\longrightarrow} [1;m]
  \qquad
  \forall i \in [1;n].\ \vartheta_i \rhd A_i \subty B_{\varphi(i)}
}{
  (\varphi, (\vartheta_i)_{i \in [1;n]}) \rhd (A_1 \otimes \dots \otimes A_n) \subty (B_1 \otimes \dots \otimes B_m)
}
%

Let \( \Gamma \vdash M : A \) and \( \Gamma' \vdash M' : A' \) and \( (\Phi, \varphi) \rhd (\Gamma \vdash A) \subty (\Gamma' \vdash A') \).  The relation \( (\Phi, \varphi) \rhd (\Gamma \vdash M : A) \sqsubseteq (\Gamma' \vdash M' : A') \) is defined by induction on derivations:
%
\infrule{
  (\Phi[x \mapsto \psi], \varphi) \rhd (\Gamma, x : \vec{A} \vdash M : B) \sqsubseteq (\Gamma', x : \vec{A}' \vdash M' : B')
}{
  (\Phi, (\psi, \varphi)) \rhd (\Gamma \vdash \lam x. M : \vec{A} \multimap B) \sqsubseteq (\Gamma' \vdash \lam x. M' : \vec{A}' \multimap B')
}
\infrule{
  \exists \vartheta \rhd \vec{B} \subty \vec{B}' \\
  (\Phi_1, (\vartheta, \varphi)) \rhd (\Gamma_1 \vdash M : \vec{B} \multimap A) \sqsubseteq (\Gamma'_1 \vdash M' : \vec{B}' \multimap A')
  \\
  (\Phi_2, \vartheta) \rhd (\Gamma_2 \vdash T : \vec{B}) \sqsubseteq (\Gamma'_2 \vdash T' : \vec{B}')
}{
  (\Phi_1 \wedge \Phi_2, \varphi) \rhd (\Gamma_1 \wedge \Gamma_2 \vdash M\,T : A) \sqsubseteq (\Gamma'_1 \wedge \Gamma'_2 \vdash M'\,T' : A')
}
\infrule{
  \forall i \in [1;n].\ (\Phi_i, \varphi_i) \rhd (\Gamma_i \vdash M_i : A_i) \sqsubseteq (\Gamma'_{\vartheta(i)} \vdash M'_{\vartheta(i)} : A'_{\vartheta(i)})
}{
  (\bigwedge_{i = 1}^{n} \Phi_i, (\vartheta, (\varphi_i)_{i \in [1;n]})) \\
  \rhd (\bigwedge_{i = 1}^n \Gamma_i \vdash \langle M_i \rangle_{i = 1}^{n} : \bigwedge_{i = 1}^{n} A_i) \sqsubseteq (\bigwedge_{j = 1}^{m} \Gamma'_j \vdash \langle M'_j \rangle_{j = 1}^{m} : \bigwedge_{j = 1}^{m} A'_j)
}
%

\subsection{Equivalence between games and terms}

\( F : {\mathbb{I}\mathbb{B}} \to \mathbb{I} \) and \( G : \mathbb{I} \to {\mathbb{I}\mathbb{B}} \) such that \( G F = \ident \).  (Hence \( F \) is faithful and \( G \) is full.  In fact \( F \) is full and faithful.)

Furthermore the equivalence can commute with projections in the following sense:
\begin{itemize}
\item \( G \circ \pi = \pi \circ G : {\mathbb{I}\mathbb{B}} \to {\mathbb{P}} \).
\item \( \alpha : \pi \circ F \stackrel{\cong}{\longrightarrow} F \circ \pi : {\mathbb{I}} \to {\mathbb{B}} \).
\end{itemize}
For the third projection (the \( \Component{A, C} : \CIntr{A, B, C} \to \CPlay{A, C} \) and its term-side counterpart), both natural isomorphisms are identities.




